AggFT: Low-Cost Fault-Tolerant Smart Meter Aggregation with Proven Termination and Privacy

Smart meter data aggregation protocols have been developed to address rising privacy threats against customers' consumption data. However, these protocols do not work satisfactorily in the presence of failures of smart meters or network communication links. In this paper, we propose a lightweight and fault-tolerant aggregation algorithm that can serve as a solid foundation for further research. We revisit an existing error-resilient privacy-preserving aggregation protocol based on masking and improve it by: (i) performing changes in the cryptographic parts that lead to a reduction of computational costs, (ii) simplifying the behaviour of the protocol in the presence of faults, and showing a proof of proper termination under a well-defined failure model, (iii) decoupling the computation part from the data flow so that the algorithm can also be used with homomorphic encryption as a basis for privacy-preservation. To best of our knowledge, this is the first algorithm that is formulated for both, masking and homomorphic encryption. (iv) Finally, we provide a formal proof of the privacy guarantee under failure. The systematic treatment with strict proofs and the established connection to graph theory may also serve as a starting point for possible generalizations and improvements with respect to increased resilience.

==> RelatedWork.tex <==
Secure and Privacy-Friendly Local Electricity Trading and Billing in Smart Grid \cite{abidin2018secure}: 
This paper two protocols for the secure computation of local electricity trading and billing. They do so by utilizing the existing secure multiparty computation protocols. In the nutshell, the system comprises of three types of parties, namely, input providers, computational parties and output parties. Input providers outsource their secret shared data to the computational parties who conduct the MPC protocol for the intended functionality. The output is then submitted to the output parties. 
\begin{itemize}
    \item Resilience to failures (guraranteed termination without needing for example additional rounds): The communication channels are considered secure and authenticated. Also, the failure is not concerned in the system.
    \item Computational complexity: For each smat meter, n many
    \item Communication complexity:
    \item low cost for authentication due to the MACs. 
    \item Solid privacy proof: They utilize UC secure primitives whose composition is also a UC secure protocol. However, the proof is only the restatement of the UC composition theorem. 
     \item Intended adversarial model: the computation parties are honest but curious, but the input and output parties can be malicious. Nothing specific about the protection against the malicious behavior is stated as everything relies on the underlying MPC protocols that exist in the literature. 
    \item Collusion set:  all the computational parties except one. The input and output parties are non-colluding.
\end{itemize}{}



==> Security-Definition-Proof.tex <==
\subsection{Security Definition}



\subsection{Security Proof}

==> UCsecurity.tex <==
In this section the privacy guarantee of the protocol is stated and proved using the simulation-based UC security methodology.


\begin{theorem}[Privacy]
	For honest-but curious parties the aggregation scheme shown in Figure \ref{fig: algonew} has the following privacy guarantees
	\begin{enumerate}[(i)]
		\item The ideal functionality outputs either the sum of at least $\nmin$ reachable smart meters or $\bot$.
		\item The protocol $\prot$ UC-securely implements the ideal functionality.
	\end{enumerate}
\end{theorem}
\textbf{Proof:} \\
TODO


In this framework, all parties are described separately, i.e. in this case, the behavior of the $\DC$ and the smart metres $\SM$ need to be described. Note that in order to easily compare these descriptions with the new algorithm, it has already been formulated in a similar way.

\begin{algorithm}[h!]
	\setstretch{0.8}
	\tcc{Start of round t}
	Pick random $s_0$ and set $S=s_0$\\
	\While{$\Ackring$ \rm{not received from next} $\SM_j$ within $T$}
		{
		send $\langle \Lfull,t,\Lact=\{\}\rangle$ to next $\SM_j$
	}
	\lIf{$\SM_j$ \rm{was found}}
	{
	Send $\langle S \rangle$ forward to $\SM_j$
	}
%	\lIf{a $<$ b}{c}
%	\lElse{d}
	\lElse{\rm{End of round}}
	\tcc{Collect data during the round}
	\If{$\tilde{m}_{j}$ \rm{is received from} $\SM_j$ }
	{
		Store $\tilde{m}_{j}$\\
		Send $\Ackm$ to $\SM_j$
	}
	\If{$L_j$ \rm{is received from} $\SM_j$}
	{
		store $L_j$
	}
	\tcc{Finish the round}
	\If{$L_N$ \rm{is received from} $\SM_N$ \rmfamily{or round duration} $>$ $T_{\max}$}
			{
				pick $\mathrm{best} = \argmax_{j}\vert L_j \vert$\\
				send $\AckL$ to $\SM_{\mathrm{best}}$\\
				Calculate Average $A_t = \left[\sum\limits_{j \in L_{\mathrm{best}}} \tilde{m}_{j} - \PRFj \right]- S_{\mathrm{best}}$
			}
	\caption{$\DC$ algorithm during aggregation}  \label{fig: algoDC}
\end{algorithm}




\begin{algorithm}[h!]
	\setstretch{0.8}
		\If{$\langle \Lfull,t,\Lact=\{\}\rangle$ \rm{is received from}  $\SM_i$}
		{
		Send $\Ackring$ back to $\SM_i$	
		}
		\If{ $\langle S \rangle$  \rm{is received from}  $\SM_i$}
		{
		Store $S$.\\
		Pick random $s_j$\\
		Set $\tilde{m}_{j}= m_{j,t}+s_{j} + \PRFj \mod k$\\
		Send $\tilde{m}_{j}$ to $\DC$
		
		Wait until ($\Ackm$ \rm{received from} $\DC$) or (duration$\geq T$)\\
		\If{$\Ackm$ \rm{received from} $\DC$}
		{
		Set $S= S+s_{j} + \PRFj \mod k$\\
		Set $\Lact=\Lact \cup \{i\}$\\
		\If{$\vert \Lact \vert \geq \nmin$}
		{
			Send $\mathrm{L}_j:=\Lact$ to $\DC$\\
		}		
		}
		\While{$\Ackring$ \rm{not received from next} $\SM_i$}
		{
			send $\langle \Lfull,t,\Lact \rangle$ to next $\SM_i$
		}
	}
		\If{$\AckL$ \rm{received from} $\DC$}
		{
			Send $\langle S \rangle$ to $\DC$
		}
	
\caption{$\SM$ algorithm}  \label{fig: algoSM}
\end{algorithm}



==> complicatedAlgo.tex <==
\subsection{Improved algorithm}

The improved algorithm is described in algorithm 2 and the individual messages sent for the sample network (Figure \ref{fig:exNetwork0}) are shown in Figure \ref{fig:exampleAlgo}.  The normal operation is illustrated by concentrating on smart meter $\SM_2$. $\SM_1$ contacts $\SM_2$ with message 5 including the sending lists. This message \textit{activates} smart meter $\SM_2$ which immediately sends an Ack-message 6 back to the $\SM_1$. Due to the assumption of static link failures during a round the Ack-signal gets back to $\SM_1$ and $\SM_1$ can successfully send the sum of shares $S$ to $\SM_2$ with message 7. Now $\SM_2$ takes over and $\SM_1$ can get inactive. $\SM_2$ tries to send its masked value to the $\DC$ (8). The $\DC$ sends an Ack back, so $\SM_2$ knows that the $\DC$ has its masked value and that it can \textit{contribute} to the aggregate. Therefore it adds itself to the list of contributing smart meters $\Lact$ and adds its share to the sum of shares $S$ (lines 28 and 29). Then $\SM_2$ in turn tries to contact the next smart meter. 

\input{tikz/algoIntermediate.tex}

% example algorithm
\begin{figure}
	\centering
	\input{tikz/tikzFigExampleAlgo.tikz}
\caption{Example demonstrating how the algorithm proceeds along the network. Dashed arrows are ack-signals that notifies a successful reception of a message. Note that there is no ack for the receipt of  message 7 because the sender already knows that the link works due to ack-signal 6. Note that $\SM_4$ does not update $S$ ($S_4=S_2$), because $\SM_4$ can not contribute to the sum due to a missing connection to the $\DC$. $\SM_4$ knows this because it gets no ack-signal from the $\DC$. $\SM_6$ is active, but a dead end: it has no connection to any subsequent smart meter and no connection to the $\DC$. Therefore it tells $\SM_5$, that the round ends. $SM_5$ tells the $\DC$ that the round ends and provides the list of contributing smart meters and the sum of shares $S$.}
\label{fig:exampleAlgo}
\end{figure}


Note that the initial contact procedure starting at the $\DC$ is analogous to this situation. The only difference is that message 4 superfluous since the $\DC$ in this case has also played the role of the contacting smart meter. If the link to the next smart meter is not working, no Ack gets back within $\Delta t$ and the active smart meter knows that it needs to skip this smart meter. 

Thus $\SM_3$ successfully contacts $\SM_4$ which gets active. However, $\SM_4$ has no working link to the $\DC$. Due to the missing Ack-signal it knows that it can not \textit{contribute} to the aggregate (skip of updates in lines 28 and 29). So this case can not only be detected but handled in a natural way.

When it comes to finishing the round, in the standard case the next party is the $\DC$ (line 37), which gets the end-of-round-message $E_t$ and the sum of shares, if the number of contributing smart meters exceeds $\nmin$. As discussed before, in the example the last smart meter $\SM_6$ has no connection to the $\DC$. Therefore it sends the end-of-round-message $E_t$ to $\SM_5$ which is the last contributing smart meter and therefore sends the data to the $\DC$ as in the standard case (line 49). If it is not contributing one more step back along the path is needed until a contributing smart meter 
(or in the worst case the $\DC$) is found.

The $\DC$ then finishes the round by subtracting the received sum of shares (if obtained) and the PRFs which he can compute himself using the shared key $k_i$. Due to the removal of the homomorphic hashes the corresponding checks are of course not needed any more.

As a quick summary the path along which the parties successfully contact each other is shown in Figure \ref{fig:exampleNetwork}. All but smart meter $\SM_3$ which could not be contacted by $\SM_2$ were active, but only smart meters 1,2 and 5 contribute, the end-of-round-message was transmitted by $\SM_5$.


\textbf{TODO: check the discussion of the improved algorithm,  state that there also guarantees exist, but they are shown in the appendix}

% connections for example
% \def\xDC{4}
% \def\yscale{0.8}
% \def\bend{50}
% \def\bendz{15}




% \begin{figure}
% 	\centering
% 	\input{tikz/tikzNetwork0.tikz}
% \caption{Example network consisting of 6 smart meters and the data concentrator used to demonstrate the algorithms and arising problems. The connections between the nodes are the links that work at round $t$.}
% \label{fig:exNetwork0}
% \end{figure}





\begin{figure} 
	\centering
	\input{tikz/tikzFigNetwork.tikz}
\caption{Example network showing the smart meters as nodes on the left and the $\DC$ at the right and all connections working at aggregation round $t$. Round smart meter nodes will be active in the algorithm, but only nodes filled with green color will contribute to the sum. White, round nodes do not contribute to the sum due to the missing link to the $\DC$. Red, rectangular nodes do not contribute to the sum since they are never active during the algorithm. As a result, some connections (marked as dashed, gray) exist but are not used during aggregation round $t$.}
\label{fig:exampleNetwork}
\end{figure}



% \begin{figure}
% 	\centering
% 	\input{tikz/tikzNetwork2.tikz}
% \label{fig:exNetwork2}
% \caption{Example network for simpler algorithm showing the smart meters as nodes on the left and the $\DC$ at the right and all connections working at aggregation round $t$. Red, rectangular nodes do not contribute to the sum due to the missing link to the $\DC$. They are never active during the algorithm and connections to these nodes (marked as dashed, gray) exist but are not used during aggregation round $t$. Only round smart meter nodes may be active in the algorithm. Due to its isolation from other potentially active smart meters smart meter 4 can never contribute to the aggregate although it is linked to the $\DC$.}
% \end{figure}



==> correctness.tex <==

Now the algorithm is analyzed with specified privacy preserving computations. For both specifications only smart meters that get active will provide information through $S$ such that they contribute to the aggregate, inactive smart meters do not contribute. Statement (iii) of the preceding theorem also states that if less than $\nmin$ smart meters have been active only the information about the end of the round is transferred in the final message. In this case the $\DC$ does not have the needed information to compute the aggregate.
Therefore correctness of the aggregate means that the aggregate for the round obtained is the exact sum of the measurements of all the active smart meters that were active if they were at least $\nmin$. 
\[
A_t=\sum_{i \in \Lact}m_{i,t}, \quad \mathrm{if} \ | \Lact|\geq \nmin
\]
Note that honest parties follow the protocol therefore the protocol is executed as in algorithm \ref{fig: algoGeneralV02}.\\

% Note that honest (-but-curious) parties follow the protocol. There may be a collusion between parties where information is shared and additional computations are done (curious) but the protocol is executed as in algorithm \ref{fig: algoGeneralV02}.\\


\begin{theorem}[Correctness of the aggregate]
	With the same assumptions as in the preceding theorem and the assumption that all parties honestly follow the protocol and at least $\nmin$ smart meters were active in round $t$ the following holds\\
	(i) Replacing in algorithm \ref{fig: algoGeneralV02} the computations in lines 2, 6, 10 and 29 by masking as in Section \ref{sec: generalizeComputation}, the aggregate is correctly calculated by the $\DC$.\\
	(ii) Replacing in algorithm \ref{fig: algoGeneralV02} the computations in lines 2, 6, 10 and 29  by homomorphic encryption as in Section \ref{sec: generalizeComputation}, the aggregate is correctly calculated by the $\DC$.

% (ii) Calculation of the aggregate: When replacing the corresponding computations by using either masking or homomorphic encryption as in Section \ref{sec: generalizeComputation} the following holds: An aggregate can only be calculated by the $\DC$, if the number of contributing smart meters exceeds $\nmin$. Otherwise the algorithm terminates the round. This termination is not triggered by the $\DC$ but by the smart meters. The aggregate obtained is the exact sum of the measurements of all the $\geq \nmin$ smart meters that were active during this round.\\

\end{theorem}
\begin{proof}
\input{proofs/proofCorrectnessFull}
%\input{proofs/proofCorrectnessShort}
\end{proof}

% \begin{proof}
% %\textbf{Proof:}\\
% (i) In line 2, the $\DC$ gets the masked values of all smart meters in $\Lcand$. Since all active smart meters are in $\Lcand$ (lines 7 and 15, respectively), it consequently has the masked values $\tilde{m}_{i}= m_{i,t}+s_{i} + \PRF{j} \mod k$ of all active smart meters. Since in line 10 only active smart meters act,  $S=s_0+\sum\limits_{i \in \Lact} s_i$ due to the corresponding substitutions in lines 6 and line 10. 
% As shown in in the previous theorem, only if at least $\nmin$ smart meters have been active, this $S$ is sent to the $\DC$ in line 26. The correctness then follows from inserting all this in $A_t$ and modular arithmetics which allows the summations to be done in arbitrary order. It can be then seen that all the terms except the sum of the measurements cancel each other out.
% % \begin{eqnarray*}
% %      A_t & = & -S-s_0+\sum\limits_{i \in \Lact} \tilde{m}_{i} - \sum\limits_{i \in \Lact} \PRFj \mod k\\
% %      & = & -(s_0+\sum\limits_{i \in \Lact} s_i)-s_0\\
% %     &  & +\sum\limits_{i \in \Lact} \left( m_{i,t}+s_{i} +\PRFj \mod k\right) \\
% %     & &  - \sum\limits_{i \in \Lact} \PRFj \mod k\\
% % \end{eqnarray*}     


% (ii) For homomorphic encryption, in line 2, the $\DC$ gets the indices of all smart meters so that it can determine $\Lcand$ needed for the algorithm. Analogously to masking, through the calculations in line lines 6 and 10 $S$ is now the product $E_{pk}(0)\cdot \prod\limits_{i \in \Lact} 
% \cdot E_{pk}(m_{i,t})$. The correctness follows from inserting this in $A_t$ and the homomorphic property of the encryption scheme and that the fact that  $\DC$ (only the $\DC$) has the secret key 
% \begin{eqnarray*}
% D_{sk}(S)&=&D_{sk}\left(E_{pk}(0)\cdot \prod_{i \in \Lact}S_i\right)\\
% &=&D_{sk}\left(E_{pk}(0)\cdot \prod_{i \in \Lact}E_{pk}(m_{i,t})\right)=\sum_{i \in \Lact}m_{i,t}\\
% \end{eqnarray*} 

% % $\square$
%  \end{proof}
In contrast to masking, when using homomorphic encryption in line 2 the $\DC$ gets no information that is needed for the computation of the aggregate, these messages are however needed for the determination of $\Lcand$ which is needed for the algorithm.

==> proofs/BackupPrivacyProofHomomorphic.tex <==
%In the reduction, $B$ acts as the challenger for the unlinkability game and as the adversary for the CPA game of the encryption scheme. $B$ gets the encryption public key $pk$ from the CPA challenger and hands it to the adversary as part of the intialization phase. $\A$ outputs $m_0, m_1$ as the measurements of the honest smart meters $SM_{i^*}$ and $SM_{j^*}$.  $B$ needs to leverage the success power of $\A$  to get to win the CPA game due to which it proceeds as follows. $B$ crafts two message vectors of the following forms $\overrightarrow{v_0}=(m_0,m_1)$ and $\overrightarrow{v_1}=(m_1,m_0)$. $\overrightarrow{v_0}$  and $\overrightarrow{v_1}$  signify two different possible assignments of $m_0$ and $m_1$ to the challenged smart meters, i.e. the first and the second items in each vector represent the respective measurements of $SM_{i^{*}}$ and $SM_{j^{*}}$. $B$ submits $\overrightarrow{v_0}$ and $\overrightarrow{v_1}$ to the CPA challenger as part of the CPA challenge phase. In return, the CPA challenger picks a random bit $b$, encrypts one of the input vectors accordingly and submits the result to $B$. Let $\overrightarrow{C_b}=(c_b,c_{\hat{b}})$ denote the resultant cipher vector. Notice that if $b==0$ then $\overrightarrow{C_b}$ is the encryption of $\overrightarrow{v_0}$, and otherwise it is the encryption of $\overrightarrow{v_1}$. $B$ uses $c_b$ and $c_{\hat{b}}$ as the measurements of $SM_{i^*}$ and $SM_{j^*}$, respectively. In fact, by  asking the CPA challenger to randomly encrypt one of the message vectors, $B$ deliberately delegates the task of the measurement assignment to the CPA challenger. As such, the choice of $b$ is not under the control of $B$ and instead, it is related to the CPA game. Therefore, if $\A$ manages to figure out which measurement is assigned to which smart meter (to distinguish between $\overrightarrow{v_0}$ and $\overrightarrow{v_1}$), $B$ can also figure out which message vector was encrypted by the CPA challenger and hence can win the CPA game. 

%The adversary decides on the arrangement of smart meters as well as the the network failure model $G'$, which ultimately influences the list of contributing  smart meters, i.e. $\Lact$ (recall that $\Lact$ certainly includes the challenged smart meters, as otherwise the adversary loses). $\A$ can exploit its control over $N-2$ smart meters, $L$, and  $\Lact$ in two possible ways: 1) $\A$ places  $SM_{i^*}$ and $SM_{j^*}$ as each other's immediate neighbors in $\Lact$,  in which case $\A$ gets to obtain the aggregate of $SM_{i^*}$ and $SM_{j^*}$ encrypted measurements, i.e. $Enc_{pk}(m_b+m_{\hat{b}})$. 2) Otherwise, $\A$, playing the immediate neighbors of challenged smart meters in $\Lact$, obtains the individual encrypted measurements of $SM_{i^*}$ and $SM_{j^*}$, i.e. $c_b=Enc_{pk}(m_b)$ $c_{\hat{b}}=Enc_{pk}(m_{\hat{b}})$. The former case does not carry any information about $b$ (since it is independent of $b$), whereas the latter case might lead to some leakage about $b$ if the deployed encryption scheme is not CPA-secure, i.e. if $\A$ can distinguish between the messages encapsulated in $c_{b}$ and $c_{\hat{b}}$ (in other words, to distinguish between  $\overrightarrow{v_0}$ and $\overrightarrow{v_1}$). $\A$ outputs its guess as $b'$, which $B$ sends directly to the CPA challenger. If $\A$ has non-negligible advantage to win the unlinkability game so does $B$ in the CPA-game. 

% \begin{comment}
% \textbf{Formal proof}
% \begin{enumerate}

%     \item The initialization part of the aggregation protocol is run. The challenger is given the encryption key $pk$ from the CPA challenger.  The challenger gives the network graph $G=(V, E)$ to the adversary. 
%     \item The adversary $\A$ outputs a pair of measurements $m_0, m_1$  within the measurement domain. $\A$ also determines two smart meters $SM_{i^*}$ and $SM_{j^*}$ (the challenged smart meters) to which the given measurements shall be randomly assigned. The adversary also specifies the measurements of all the remaining smart meters, i.e., $MList=\{(SM_i, m_i)\}$ for $i\notin \{ i^{*},j^{*}\}$. The adversary sends out the network failure model $G'=(V', E')$ as well as an ordered list $L=(DC, SM_1, SM_2,\cdots, SM_N, DC)$ that indicates the arrangements of smart meters in the aggregation protocol.
%     \item The challenger checks that $L$ starts and ends with $DC$, and contains all the smart meters exactly once. The challenger also checks that the challenged smart meters $SM_{i^*}$ and $SM_{j^*}$ can contribute to the aggregation in the network failure model $G'=(V', E')$ provided by the adversary, and that it is a valid failure model ($V' = V \wedge E' \subseteq E$). If any of the checks fail, the challenger stops and the adversary loses the game with the game’s output being $0$. Otherwise (if all checks succeed), the challenger assigns the measurements of smart meters according to $MList$.
    
%     For the  challenged smart meters, $B$ proceeds as follows (in this step, $B$ needs to leverage the success power of $\A$ to win the CPA game). $B$ crafts two message vectors of the following forms $\overrightarrow{v_0}=(m_0,m_1)$ and $\overrightarrow{v_1}=(m_1,m_0)$. $\overrightarrow{v_0}$  and $\overrightarrow{v_1}$  signify two different possible assignments of $m_0$ and $m_1$ to the challenged smart meters, i.e. the first and the second items in each vector represent the respective measurements of $SM_{i^{*}}$ and $SM_{j^{*}}$. $B$ submits $\overrightarrow{v_0}$ and $\overrightarrow{v_1}$ to the CPA challenger as part of the CPA challenge phase. In return, the CPA challenger picks a random bit $b$, encrypts one of the input vectors accordingly and submits the result to $B$. Let $\overrightarrow{C_b}=(c_b,c_{\hat{b}})$ denote the resultant cipher vector. Notice that if $b==0$ then $\overrightarrow{C_b}$ is the encryption of $\overrightarrow{v_0}$, and otherwise it is the encryption of $\overrightarrow{v_1}$. $B$ uses $c_b$ and $c_{\hat{b}}$ as the measurements of $SM_{i^*}$ and $SM_{j^*}$, respectively. 
%     \item The challenger and the adversary proceed with the steps of the aggregation protocol using the network failure model provided by the adversary. 
%     \item $\A$ outputs its guess as $b'$, which $B$ sends directly to the CPA challenger.
% \end{enumerate}

% Notice that at step 3, when $B$ asks the CPA challenger to randomly encrypt one of the message vectors, $B$ deliberately delegates the task of the measurement assignment to the CPA challenger. As such, the choice of $b$ is not under the control of $B$ and instead, it is related to the CPA game. Therefore, if $\A$ manages to figure out which measurement is assigned to which smart meter (to distinguish between $\overrightarrow{v_0}$ and $\overrightarrow{v_1}$), $B$ can also figure out which message vector was encrypted by the CPA challenger and hence can win the CPA game. 

% The view of adversary in the game is determined by the arrangement of smart meters as indicated in $L$  as well as the the network failure model $G'$, which ultimately influences the list of contributing  smart meters, i.e. $\Lact$ (recall that $\Lact$ certainly includes the challenged smart meters, as otherwise the adversary loses). $\A$ can exploit its control over $N-2$ smart meters, $L$, and  $\Lact$ in two possible ways: 1) $\A$ places  $SM_{i^*}$ and $SM_{j^*}$ as each other's immediate neighbors in $\Lact$,  in which case $\A$ gets to obtain the aggregate of $SM_{i^*}$ and $SM_{j^*}$ encrypted measurements, i.e. $Enc_{pk}(m_b+m_{\hat{b}})$. 2) Otherwise, $\A$, playing the immediate neighbors of challenged smart meters in $\Lact$, obtains the individual encrypted measurements of $SM_{i^*}$ and $SM_{j^*}$, i.e. $c_b=Enc_{pk}(m_b)$ $c_{\hat{b}}=Enc_{pk}(m_{\hat{b}})$. The former case does not carry any information about $b$ (since it is independent of $b$), whereas the latter case might lead to some leakage about $b$ if the deployed encryption scheme is not CPA-secure, i.e. if $\A$ can distinguish between the messages encapsulated in $c_{b}$ and $c_{\hat{b}}$ (in other words, to distinguish between  $\overrightarrow{v_0}$ and $\overrightarrow{v_1}$).

% $\square$

% %When using homomorphic encryption as described in Section \ref{sec: generalizeComputation}, the same maximum collusion sets arise but now both guarantees are computationally hard (Figure \ref{fig:privVisu2}). Again, if the $\DC$ could collude with $\SM_2$ and calculate $D_{sk}(S_1)=m_{1,t}$ (\textbf{TODO change substitution S0=E(0)? in Line 6 by something else?}). The smart meters can in turn not infer information from $S_1$ about $m_{1,t}$, since they do not own the secret key $sk$. 


% % In the reduction, $B$ acts as the challenger for the unlinkability game and as the adversary for the CPA game of the encryption scheme. $B$ gets the encryption public key $pk$ from the CPA challenger and hands it to the adversary as part of the intialization phase. $\A$ outputs $m_0, m_1$ as the measurements of the honest smart meters $SM_{i^*}$ and $SM_{j^*}$.  $B$ needs to leverage the success power of $\A$  to win the IND-CPA game due to which it proceeds as follows. $B$ crafts two message vectors of the following forms $\overrightarrow{v_0}=(m_0,m_1)$ and $\overrightarrow{v_1}=(m_1,m_0)$. $\overrightarrow{v_0}$  and $\overrightarrow{v_1}$  signify two different ordered assignments of $m_0$ and $m_1$ to $SM_{i^{*}}$ and $SM_{j^{*}}$, respectively. $B$ outputs $\overrightarrow{v_0}$ and $\overrightarrow{v_1}$ as part of the CPA challenge phase and obtains a cipher vector $\overrightarrow{C_b}=(c_b,c_{\hat{b}})$ where $b$ is the bit selected randomly by IND-CPA challenger.
% % Notice that if $b==0$ then $\overrightarrow{C_b}$ is the encryption of $\overrightarrow{v_0}$, and otherwise it is the encryption of $\overrightarrow{v_1}$. 
% % $B$ uses $c_b$ and $c_{\hat{b}}$ as the measurements of $SM_{i^*}$ and $SM_{j^*}$, respectively. 

% % In fact, by  asking the CPA challenger to randomly encrypt one of the message vectors, $B$ deliberately delegates the task of the measurement assignment to the CPA challenger. As such, the choice of $b$ is not under the control of $B$ and instead, it is related to the CPA game. Therefore, if $\A$ manages to figure out which measurement is assigned to which smart meter (to distinguish between $\overrightarrow{v_0}$ and $\overrightarrow{v_1}$), $B$ can also figure out which message vector was encrypted by the CPA challenger and hence can win the CPA game. 



% \subsubsection{Proof of Theorem \ref{thm_homo}.(i)}
% In the reduction, $B$ acts as the challenger for the unlinkability game and as the adversary for the CPA game of the encryption scheme. $B$ gets the encryption public key $pk$ from the CPA challenger and hands it to the adversary as part of the intialization phase. $\A$ outputs $m_0, m_1$ as the measurements of the honest smart meters $SM_{i^*}$ and $SM_{j^*}$.  $B$ needs to leverage the success power of $\A$  to win the IND-CPA game due to which it proceeds as follows. $B$ crafts two message vectors of the following forms $\overrightarrow{v_0}=(m_0,m_1)$ and $\overrightarrow{v_1}=(m_1,m_0)$ where each vector signifies an ordered assignment of $m_0$ and $m_1$ to $SM_{i^{*}}$ and $SM_{j^{*}}$, respectively. $B$ outputs $\overrightarrow{v_0}$ and $\overrightarrow{v_1}$ as part of the CPA challenge phase and obtains a cipher vector $\overrightarrow{C_b}=(c_b,c_{\hat{b}})$ where $b$ is the bit selected randomly by IND-CPA challenger.
% %Notice that if $b==0$ then $\overrightarrow{C_b}$ is the encryption of $\overrightarrow{v_0}$, and otherwise it is the encryption of $\overrightarrow{v_1}$. 

% $B$ uses $c_b$ and $c_{\hat{b}}$ as the measurements of $SM_{i^*}$ and $SM_{j^*}$, respectively. 

% %In fact, by  asking the CPA challenger to randomly encrypt one of the message vectors, $B$ deliberately delegates the task of the measurement assignment to the CPA challenger. As such, the choice of $b$ is not under the control of $B$ and instead, it is related to the CPA game. Therefore, if $\A$ manages to figure out which measurement is assigned to which smart meter (to distinguish between $\overrightarrow{v_0}$ and $\overrightarrow{v_1}$), $B$ can also figure out which message vector was encrypted by the CPA challenger and hence can win the CPA game. 

% The adversary decides on the arrangement of smart meters as well as the the network failure model $G'$, which ultimately influences the list of contributing  smart meters, i.e. $\Lact$ (recall that $\Lact$ certainly includes the challenged smart meters, as otherwise the adversary loses). 

% The view of $\A$ toward the challenged smart meters depends on the arrangement of smart meters: 

% 1)  $SM_{i^*}$ and $SM_{j^*}$ are each other's immediate neighbors in $\Lact$,  in which case $\A$, controlling the non-challenged smart meters, gets to obtain the aggregate of $SM_{i^*}$ and $SM_{j^*}$ encrypted measurements, i.e. $Enc_{pk}(m_b+m_{\hat{b}})$. 
% 2) Otherwise, $\A$, playing the immediate neighbors of challenged smart meters in $\Lact$, obtains the individual encrypted measurements of $SM_{i^*}$ and $SM_{j^*}$, i.e. $c_b=Enc_{pk}(m_b)$ $c_{\hat{b}}=Enc_{pk}(m_{\hat{b}})$.

% The former case does not carry any information about $b$ (since it is independent of $b$), whereas the latter case might lead to some leakage about $b$ if the deployed encryption scheme is not CPA-secure, i.e. if $\A$ can distinguish between the messages encapsulated in $c_{b}$ and $c_{\hat{b}}$ (in other words, to distinguish between  $\overrightarrow{v_0}$ and $\overrightarrow{v_1}$).

% $\A$ outputs its guess as $b'$, which $B$ sends directly to the CPA challenger. If $\A$ has non-negligible advantage to win the unlinkability game so does $B$ in the CPA-game. 


% %\input{proofs/PrivacyProofHomomorphicFull}

 


% \begin{comment} 

% The algorithm contains two parts which aim at loosening the HBC assumption.
% First, note that we proved that the end of the round is determined by the smart meters and not by the $\DC$. While this makes no difference for an honest $\DC$, this limits the possibilities for a dishonest $\DC$: for example for masking the $\DC$ may try to send an $\EOR$ signal to the 2 neighboring smart meters of $\SM_i$, ($\SM_{i-1}$ and $\SM_{i+1}$) in order to get the final messages. From these messages $m_i$ can be simply computed from $m_i=\tilde{m_i}-(\SM_{i+1}-\SM_{i-1}$. An analogous method works for homomorphic encryption.\\
% Second, as already discussed in section \ref{sec:improveSecurity} the usage of the round-dependent PRFs prevents external eavesdroppers of the communication links from inferring useful information.
% \end{comment}

% % There are some protocols with higher privacy guarantees: there, nearly all smart meters could collude with $\DC$ (for example the low overhead protocol of Kursawe). However, in these protocols typically each pair of smart meters $i$ and $j$ share a common key $k_{ij}(t)$. One smart meter adds $k_{ij}(t)$ it to its measurement, the other one subtracts it so these shares sum up to zero. This pairwise addition and subtraction is done for all pairs. While this can be done effectively and has a higher privacy guarantee, it is not fault tolerant. If a single smart meter fails, the sum of shares do not cancel each other and the aggregate is useless.



% \subsubsection{Proof of Theorem \ref{thm_homo}.(ii)}
% The privacy proof against $DC$ is information-theoretic. This because the view of $\A$ toward the challenged smart meters is limited to their sum of measurements regardless of how adversary influences the network failure model $G'$ and the arrangement list $L$ (under any $G'$ and $L$, both challenged smart meters are guaranteed to be part of the aggregation due to step 3 of the $\Unlink$). $\A$ obtains the final aggregate  $A_t = m_b + m_{\hat{b}}+ \sum_{i \in \Lact/\{SM_{i^*},SM_{j^*}\}} m_{i,t}$  and can narrow it down to $m_b + m_{\hat{b}}$ by subtracting the measurements of non-challenged smart meters. However, the value of $m_b + m_{\hat{b}}$ is independent of $b$ thus conveys no information for breaking $\Unlink$ game. $\square$

% %as explained next. During the unlinkability game, the adversary decides on the exact measurements of the non-challenged smart meters, the measurements of challenged smart meters $m_0$ and  $m_{1}$ and  the network failure model $G'$ which influences the list $\Lact$ i.e., the contributing smart meters. The challenger randomly assigns $m_0$ and  $m_{1}$ to the challenged smart meters and at the end, $\A$ obtains the final aggregate  $A_t = m_b + m_{\hat{b}}+ \sum_{i \in \Lact/\{SM_{i^*},SM_{j^*}\}} m_{i,t}$ (recall that $\Lact$ embodies the challenged smart meters due to the checks done at step 3). $\A$ knows the measurements of the non-challenged smart meters i.e., $ \Lact/\{SM_{i^*},SM_{j^*}\}$, thus it can extract the aggregate of challenged smart meters' measurements from $A_t$ which is $A_t- \sum_{i \in \Lact/\{SM_{i^*},SM_{j^*}\}} m_{i,t}= m_b + m_{\hat{b}}$. However, the value of $m_b + m_{\hat{b}}$ is independent of choice $b$ and the adversary obtains no useful information from its interaction with the challenger to yield a correct guess $b'$.

% % \begin{align}
% %     A_t - \sum_{i \in \Lact/\{SM_{i^*},SM_{j^*}\}} m_{i,t}  & = \\
% %     \sum_{i \in \Lact} m_{i,t}- \sum_{i \in \Lact/\{SM_{i^*},SM_{j^*}\}} m_{i,t} & = \\
% %     \sum_{SM_{i^*},SM_{j^*}}m_{i,t} = m_b + m_{\hat{b}}
% % \end{align}

% \end{comment}


==> proofs/BackupPrivacyProofMasking.tex <==


% \begin{comment}

% \begin{enumerate}
%     \item The challenger is given a vector of two values $\overrightarrow{S} =<s_0,s_1>$ from the outside PRG indistinguishability game. The initialization part of the aggregation protocol is run. The adversary sends out an ordered list $L=(DC,SM_1,SM_2,\cdots, SM_N, DC)$. 
%     \item The adversary $\A$ outputs a pair of measurements $m_0 , m_1$  within the measurement domain. $\A$ also determines two smart meters $SM_{i^*}$ and $SM_{j^*}$ to which the given measurements shall be randomly assigned. 
%     \item  The challenger draws a random bit $b \in \{ 0, 1 \}$ and assigns $m_b$ to $SM_{i^*}$ and $m_{\hat{b}}$ to $SM_ {j^*}$.
%     \item The challenger and the adversary proceed with other steps of the aggregation protocol. 
%     \begin{enumerate}
%         \item $B$ attempts the execution of line 2 of the aggregation. As such, $B$ queries $\A$'s network model oracle for $(SM_i,DC)$ for $i\in\{1,\cdots,N\}$ and obtains the link $status$ and stores it i.e., $Network.insert(SM_i,DC,status)$. If the status is 1, then $B$ sends the masked measurements $\tilde{m_i} $ to $\A$, otherwise does not. For $SM_{i^*}$ or $SM_{j^*}$, if they have active links with $DC$, $B$ uses $s_0$ and $s_1$ to mask their measurements as shown below, \begin{align}
%             \tilde{m_{i^*}}= m_{i^{*},t}+s_{b} + \PRF{i^{*}} \mod k \nonumber \\
%             \tilde{m_{j^*}}= m_{j^{*},t}+s_{\hat{b}} + \PRF{j^{*}} \mod k 
%         \end{align}
%         \item $DC$ outputs $S$ alongside with $\Lcand$, and $\Lact$ to $SM_i$ (which is controlled by the $B$  (lines 6--8 of Algorithm \ref{fig: algoGeneralV02}). $B$ sends an $\Ackring$ to $\A$.
%         \item For each smart meter in  $\Lcand$, $B$ proceeds according to lines 10-27 of Algorithm \ref{fig: algoGeneralV02}. During this part, $SM_i$ (i.e., $B$) needs to forward its calculated $S_i$ to the next reachable smart meter $SM_j\in \Lcand$ where $j>i$, as such, $B$ queries the network model oracle for $(SM_i,SM_j)$ and obtains the link $status$. The $status$ values of 1 and 0 correspond to the receipt and lack of receipt of an Ack from $SM_j$ (lines 17 and 19 of Algorithm \ref{fig: algoGeneralV02}), respectively. $B$ attempts the rest of the protocol accordingly. 
%     \end{enumerate}
%     \item $\A$ outputs her guess $b^{'}$ to $B$. The challenger checks whether the network failure model table $Netwrok$ allows $SM_{i^*}$ and $SM_{j^*}$ to successfully contribute their measurements to the final aggregate i.e., whether $SM_{i^*},SM_{j^*} \in \Lact$. If this does not hold, $B$ aborts and the output of the game is $0$ meaning $\A$ loses. Otherwise, $B$ checks whether $b==b'$, if yes, $B$ outputs 0 to the PRG indistinguishability game challenger (indicating that $s_0,s_1$ are distinguishable from truly random values), otherwise 1 (indicating that $s_0,s_1$ are indistinguishable from truly random values).
% \end{enumerate}
% Note that 
% $\A$ wins the PRG indistinguishability game if  $SM_{i^*},SM_{j^*} \in \Lact$ and 
% \begin{enumerate}
%     \item $b==b^{'}$ given that $\overrightarrow{S}$ are the output of a PRG.% In this case, $\A$ oborts.
%     \item $b \neq b^{'}$ given that $\overrightarrow{S} $ are truly random
% \end{enumerate}


% The privacy of smart meters in an aggregation protocol is preserved as long as no adversary is able to infer anything about the individual measurements. However, note privacy is in any case limited since the protocol's task is to provide the $\DC$ with the aggregate value. 
% %, so that it can be used for various purposes stated in the introduction. 
% Regardless of the underlying protocol, the aggregate itself may allow for the inference of personal information if the aggregate consists of too few values \cite{Buescher17a} (we introduced $\nmin$ for this reason). Therefore, data analysis attacks on whole load profiles such as the ones described in \cite{Buescher17a} are explicitly excluded.

% \subsection{Assumptions and Game-Based Privacy Definition}

% \textbf{Adversarial Model:}
% The communication channel between the smart meters and the $\DC$ is assumed to be secure and authenticated; %thus, the adversary is not able to eavesdrop or tamper with the communication. 
% Attackers are considered as honest but curious entities which follow the protocol but can collude and share their information to infer information about others. In addition, the adversary is granted the power to turn the links off and on i.e., to decide on the network failure model. Links are considered bidirectional and their status does not change throughout the execution of \textit{one round} of the aggregation protocol. 

% %The privacy objective is to make sure that the adversary does not infer the individual measurement of smart meters after the execution of the aggregation protocol. Clearly, as it is the goal of aggregation, the final aggregate of measurements is not privacy-sensitive and can be known by the adversary.  



% %\textbf{Proof:}\\
% %\red{TODO Sanaz: show privacy for both then masking and the homomorphic encryption variant using game-based proofs. Maybe we need the explanation and a sketch for the initial description in order to keep being below 8 pages. In the final submission, the proofs should then fit into the 2 additional pages.}





% \textbf{Formally defining unlinkability of measurements:}
% To formally capture the privacy objective under the designated adversarial model, we define the following privacy game, to be played between an adversary and a challenger, by adapting the smart meter’s data unlinkability game defined in \cite{Unterweger18b}.  The adversary controls all  colluding adversarial entities, whereas the challenger acts on behalf of the remaining honest parties.
% % We adopt the smart meter’s data unlinkability game defined in \cite{Unterweger18b}. The overall idea is a security game played between a challenger and an adversary where each control a subset of entities. The entities controlled by the challenger are honest whereas the ones controlled by the adversary are malicious. 
% The only restriction in this game is that at least two honest smart meters (out of $N$ total smart meters) are out of the adversary's control. These smart meters are called \textit{challenged smart meters}. Having less than two honest smart meters (i.e., only one honest) innately breaks the security objective, where the adversary can subtract the sum of $N-1$ known measurements from the final aggregate and extract the measurement of the remaining honest smart meter. Thus, no private aggregation protocol could satisfy such a definition with only one honest smart meter, under our adversarial model. However, even with assuming the existence of at least two honest smart meters, the adversary can pick two measurements to be assigned to the honest smart meters. This assignment is done randomly by the challenger. Thus, the adversary can even know the two measurements, but still cannot infer which measurement corresponds to which honest smart meter. The aggregation protocol preserves data unlinkability if the adversary cannot infer this assignment except with a probability \textit{negligibly} higher than a random guess. 

% We extend the data unlinkability game of  \cite{Unterweger18b} by granting  more power to the adversary as described below: 
% \begin{itemize}
%     \item The adversary additionally knows the individual measurements of any subset of the $N-2$ smart metes (in addition to the two challenged smart meters). This additional power models the real-life scenario where the adversary may have background knowledge about the electricity consumption of some of the households participating in the aggregation protocol (e.g., due to being neighbors). 
%     That knowledge might get exposed to the adversary indirectly, without the households' intention.
%     In the extended game, we therefore consider the worst-case scenario where the adversary manages to learn the measurements of all the \textit{non-challenged} smart meters as side-knowledge. Note that this does not include the secret shares or ciphertexts, which are only known for the \textit{colluding} smart meters. In the game, this is modeled by allowing the adversary to specify the individual measurements of $N-2$ non-challenged smart meters in step 2.
%     \item The adversary dictates the network failure model, i.e., the status of network links being on or off, provided that the challenged smart meters will remain contributing. %This condition is modeled by having the challenger check that restriction resulting in a losing adversary in case of not passing the check. 
%     To enable this, the network is modeled as an undirected graph $G=(V, E)$ in which $V$ is the set of vertices corresponding to the entities involved in the aggregation protocol (e.g., smart meters and $\DC$) and $E$ is the set of edges corresponding to the presence of a network link between the two connected vertices.  The adversary signifies the network failure model by outputting a sub-graph $G'=(V', E')$ of $G$ where $G'$ has an identical set of vertices (i.e., $V=V'$), but contains a subset of edges (i.e., $E'\subseteq E$).  $E'$ represents the set of network links that are working and $E \setminus E'$ indicates the offline links. Messages can be exchanged between two entities only if there is an edge connecting those entities in $E'$. Throughout the game, %the challenger needs to consult $G'$ to obtain the status of her connection with other parties. For example, 
%     when a message exchange between $SM_i$ and $SM_j$ is required, the challenger checks for an edge connecting $SM_i$ and $SM_j$ in $E'$ (i.e., whether $(SM_i,SM_j) \in E'$). Upon the existence of such an edge, a message transmission takes place; otherwise, the link is down and the challenger skips the data transmission. 

% %     The network graph $G$ and the network failure graph $G'$ corresponding to the scenario depicted in Figure \ref{fig:exNetwork0} are illustrated in Figures \ref{fig:G} and \ref{fig:GPrime}, respectively.

% In the scenario exemplified in Figure \ref{fig:exNetwork0}, the nodes of both the network graph $G$ and the network failure graph $G'$ consists of all the parties. However, while $E$ consists of all (solid and dashed) links, only the solid ones appear in $E'$; the dashed links denote the failing links in $E'\setminus E$.

% \end{itemize}  
% % \def\xDC{4}
% % \def\yscale{0.8}
% % \def\bend{50}
% % \def\bendz{15}

% % \begin{figure}[htb]
% % 	\centering
% % 	%\input{tikz/G.tikz}
% % \caption{The network graph $G$ corresponding to Figure \ref{fig:exNetwork0}.}
% % \label{fig:G}

% % \end{figure}
% % \begin{figure}[htb]
% % 	\centering
% % 	%\input{tikz/tikzNetwork2.tikz}
% % \caption{The network failure graph $G'$ corresponding to Figure \ref{fig:exNetwork0}.}
% % \label{fig:GPrime}
% % \end{figure}

% %Note that the given network failure model $G'$ is static.
% %In specific, the adversary provides a network model oracle which receives a pair of distinct parties (the index of smart meters or DC), and it returns a Boolean value asserting the liveness of the link between the queried parties. Throughout the game, the challenger needs to consult this oracle to obtain the status of her connection with other parties.  For example, when a message exchange between $SM_i$ and $SM_j$ is required, the challenger queries the network model oracle on $(SM_i, SM_j)$ and transfers the message if the query result is 1 (link is active) otherwise, the link is down and the challenger skips the data transmission. Note that the status of each link is static, i.e., either always active or down.
% The formal definition follows. 

% \textbf{Smart meters data unlinkability under chosen bi-directional network failure model $\Unlink$}:
% \begin{enumerate}
%     \item The initialization part of the aggregation protocol is run. The challenger gives the network graph $G=(V, E)$ to the adversary. 
%     \item The adversary $\A$ outputs a pair of measurements $m_0, m_1$  within the measurement domain. $\A$ also determines two smart meters $SM_{i^*}$ and $SM_{j^*}$ (the challenged smart meters) to which the given measurements shall be randomly assigned. The adversary also specifies the measurements of all the remaining smart meters, i.e., $MList=\{(SM_i, m_i)\}$ for $i\notin \{ i^{*},j^{*}\}$. The adversary sends out the network failure model $G'=(V', E')$ as well as an ordered list $L=(DC, SM_1, SM_2,\cdots, SM_N, DC)$ that indicates the arrangements of smart meters in the aggregation protocol.
%     \item The challenger checks that $L$ starts and ends with $DC$, and contains all the smart meters exactly once. The challenger also checks that the challenged smart meters $SM_{i^*}$ and $SM_{j^*}$ can contribute to the aggregation in the network failure model $G'=(V', E')$ provided by the adversary, and that it is a valid failure model ($V' = V \wedge E' \subseteq E$). If any of the checks fail, the challenger stops and the adversary loses the game with the game’s output being $0$. Otherwise (if all checks succeed), the challenger assigns the measurements of smart meters according to $MList$. For the  challenged smart meters, a random bit $b \in \{ 0, 1 \}$ is drawn and $m_b$ is assigned to $SM_{i^*}$ and $m_{\hat{b}}$ to $SM_ {j^*}$.
%     \item The challenger and the adversary proceed with the steps of the aggregation protocol using the network failure model provided by the adversary. %Throughout this interaction, for the communication between each pair of parties $P_i,P_j \in V$, the challenger checks whether $E'$ contains $(P_i,P_j)$ as an edge. Otherwise, the corresponding connection link is down.
%     %Throughout this interaction, only pairs of parties $P_i,P_j \in V$ with active links  $(P_i,P_j)\subseteq E'$ can exchange messages.
%     \item The adversary outputs her guess $b^{'}$ to the challenger. %The challenger checks whether the network failure model table $Network$ allows $SM_i$ and $SM_j$ to successfully contribute their measurements to the final aggregate. If it is the case and 
%     If $b = b^{'}$, then the adversary wins, and the output of the game is set to $1$, Otherwise, the adversary loses and the game’s output is $0$.
% \end{enumerate}

% \begin{definition}[Data Unlinkability] \label{theorem:dataUnlink}
% An aggregation protocol provides smart meters’ data unlinkability under chosen bi-directional network failure model, if for every probabilistic polynomial time (PPT) adversary $\A$, the success probability in $\Unlink$ is negligibly higher than a random guess, i.e.
% \begin{align}
%     Pr[ \Unlink = 1] \le \frac{1}{2}+ negl(\lambda) 
% \end{align}
% for some negligible probability $negl(\lambda)$, where $\lambda$ is the security parameter.
% \end{definition} 


% \textbf{Maximal collusion sets:}
% % The  privacy  guarantee  lists  allmaximal collusion sets, i.e. a subset of parties whose collusion cannot break the underlying privacy game; thus, the larger the subset the better. As the subsets are maximal, the inclusion of any further party results in the violation of the intended privacy guarantee. For example, in the case that masking protocol is utilized in  Algorithm \ref{fig: algoGeneralV02}, DC constitutes one of the maximal collusion sets, this can be verified by the fact that when $\DC$  colludes with $\SM_2$, it could compute 
% % \[
% % S_2-s_2-\mathrm{PRF}_{k_2}(t)-\mathrm{PRF}_{k_1}(t)-s_1^0 \mod k=s_1
% % \]
% % and subsequently get $m_1$ by calculating $\Tilde{m_1}-s_1-\mathrm{PRF}_{k_1}(t)  \mod k$. Thus the $\DC$ is a maximum collusion set and the aggregation protocol cannot stand an adversarial control spanning further than $\DC$. The full formal proof is presented in the rest of this section.
% The privacy guarantee lists the maximum possible corruption of various parties where privacy of the uncorrupted smart meters is still preserved. Privacy would be broken if either any more party is added or any kind of corruption is increased. Therefore, the more allowed corruption the better. 
% \begin{comment}
% % TODO may be added for the full version
% For example, for the masking protocol the DC and the \textit{fully controlled} $\SM_2$ can infer the measurement $m_1$ of $\SM_1$ by computing 
% \[
% S_2-s_2-\mathrm{PRF}_{k_2}(t)-\mathrm{PRF}_{k_1}(t)-s_1^0 \mod k=s_1.
% \]
% However, privacy can be proven to be preserved, if the adversary only knows  $\SM_2$'s measurement $m_2$, but not its shares.
% \end{comment}

% %For example, in the masking protocol depicted in   \ref{fig:privVisu1}, The maximal sets are visualized in Figure \ref{fig:privVisu1} and consist of the $\DC$ and all smart meters but the threatened one, respectively. 


% %The fact that it is computationally hard for the $\DC$ to break privacy is proven below using a game-based proof.
% %The second maximum collusion set consists of all smart meters but the one whose privacy is threatened. Of course one can not let the threatened party collude and as just shown the addition of the $\DC$ is also not possible without breaking privacy. For this maximal collusion set the privacy guarantee is even stronger than computationally hard, it is information-theoretic: the only message that contains information depending on a smart meters' measurement is sent to the $\DC$, therefore no other smart meter has any information that is in whatever sense dependent on this measurement. That's why in contrast to the $\DC$  even with infinite computational power privacy can not be broken by the smart meters. 



% %\input{tikz/privMaskingOrig}
% \input{tikz/privMaskingNew}

% %While correctness specifies what can and should be inferred, privacy deals with the inverse question, what should not be inferred. 
% \textbf{Game based privacy proofs:}
% %Computationally hard privacy with respect to the $\DC$ is proved using game-based proofs as proposed and described in \cite{Unterweger18b}. 
% Privacy with respect to the maximal collusion sets is proved using game-based proofs as described in \cite{Unterweger18b}. 
% A game-based proof is formulated as two nested games. The inner game is the game of breaking privacy stated as an unlinkability game, whereas the outer game is a common problem that is known to be \textit{(computationally) hard}. The security proof embodies a valid reduction from the inner game to the outer game  indicating that if one manages to break privacy in the inner game, then one can also win the outer game.  Since winning the outer game is known to be hard, so is the inner game.
% %Since winning this outer game is not possible in the sense of computationally hard then also winning the inner game, i.e. breaking privacy is computationally hard. The power of the attacker is indirectly described by what that the attacker is allowed to do is described in the reduction. 

% %\begin{theorem}[Privacy for masking]
% %	It is computationally hard for the $\DC$ to break privacy (yes, sloppy formulation)
% %\end{theorem}














% \subsection{ Privacy Analysis of the Masking Aggregation Protocol}
% The following theorem \ref{thm_masking} states the privacy guarantee of the protocol when masking is used: essentially, it states that the two maximal collusion sets are the ones described in Figure \ref{fig:privVisu1}. %For masking, privacy relies on the security of the underlying pseudo-random number generator. 

% \begin{taggedblock}{long}
% \input{proofs/distinguisher}
% \end{taggedblock}

% % For this protocol, we consider two maximal collusion sets 1) $DC$ and 1) a subset of $N-2$ smart meters.
% % \subsubsection{Privacy Proof against $DC$}
% % In this adversarial setting, the adversary controls $DC$ whereas the challenger runs on behalf of all the smart meters. The privacy proof, as formulated in Theorem \ref{thm_masking_dc}, relies on the security of the underlying pseudo-random number generator. 
% \begin{theorem}[Privacy of the aggregation protocol using masking] \label{thm_masking}
% Consider the protocol of Figure \ref{fig: algoGeneralV02} with privacy-preserving computations done using masking as described in Section \ref{sec:improveFlow}. The followings hold where privacy is as defined in the $\Unlink$ game:
% \begin{itemize}
%     \item[(i)] The protocol provides information-theoretic privacy against an adversary controlling $N-2$ smart meters. %Privacy of the remaining honest smart meter $\SM_j$ is information-theoretically preserved against $N-1$ colluding smart meters.
%     \item[(ii)] If the underlying PRG (used for producing masking shares) is cryptographically secure, the protocol based on masking provides privacy against an adversary controlling $\DC$.
%     \item[(iii)] Both collusion sets above are maximal.
% \end{itemize}

% \end{theorem}

% %\begin{proof}
% %\textbf{Proof: } 

% \subsubsection{Proof of Theorem \ref{thm_masking}.(i)}
% %While the proof for (i) is simple, proving (ii) is achieved using game-based proof.\\
% %(i)

% %The adversary $\A$ specifies $L$ and $G'$ (notice that since all the non-challneged smart meters are controlled by $\A$, it does not need to output $MList$ to the challenger). The combination of $L$ and $G'$ influences the smart meters adjacent to the challenged smart meters  hence the information $\A$ gets to see during its interaction with the challenged smart meters i.e., its the view in the game. Concerning the neighborhood of $SM_{i^{*}}$ and $SM_{j^{*}}$ two cases may happen:
% %1) $SM_{i^*}$ and $SM_{j^*}$ are each other's immediate neighbors in $\Lact$,  in which case $\A$ gets to obtain the aggregate of $SM_{i^*}$ and $SM_{j^*}$ masking values, i.e. $s_{i^{*}}+s_{j^{*}}$. 2) Otherwise, $\A$, playing the immediate neighbors of challenged smart meters in $\Lact$, obtains the individual masking values of $SM_{i^*}$ and $SM_{j^*}$, i.e.  $s_{i^{*}}$ and $s_{j^{*}}$. In both cases, as the adversary does not have access to the masked measurements, the masking factors does not give it any useful information


% An adversary controlling $N-2$ smart meters only gets to see the masking factors of challenged smart meters with no measurements embedded (the masked measurements are submitted to the $DC$ controlled by the challenger). As $\A$'s view is independent of the challenged smart meters measurements (hence independent of $b$), the unlinkability is preserved information-theoretically. 
% Following the preceding reasoning, the masking protocol preserves information-theoretic privacy in an extended  adversarial set consisting of $N-1$ smart meters where the privacy is defined as the inability of the adversary in distinguishing between the two possible measurements ($m_0$ and $m_1$) of the non-colluding smart meter.
% $\square$
% %The honest smart meter $SM_j$ only sends its masked value to the honest $\DC$. The dishonest $N-1$ smart meters only obtain the random share of $SM_j$, which is completely independent of its measurement. Therefore the dishonest $N-1$ smart meters lack any data that contain information about the honest smart meter's measurement, which is therefore information-theoretically secure.


% \subsubsection{Proof of Theorem \ref{thm_masking}.(ii)}
% If there exists a PPT adversary $\A$ which can win $\Unlink$, then we can construct a PPT adversary $B$ who can win the indistinguishability game of PRG. 

% \begin{comment}
% \textbf{Proof Intuition:} To provide the proof intuition, we analyze the information that $\A$ obtains during its interaction with the challenger and then show that the acquired information provides no non-negligible advantage in winning the game (otherwise the indistinguishability of the PRG can be broken). 


% The interaction of $\A$ with the challenger yields the following data (note that $\Lcand$ and $\Lact$ are determined based on $G'$ and are guaranteed to include  $SM_{i^*}$ and $SM_{j^*}$  due to the checks performed at step 3 of the game):
% \begin{align}
% \tilde{m_i} & =m_{i,t}+s_{i} + \PRF{i} \mod k  \hspace{5pt}  \forall i \in \Lcand \label{eq:mi_view}\\
% S_N &=\sum_{i \in \Lact} s_i \text{  }  \text{ where } \Lact \subseteq \Lcand \label{eq:S_view}
% \end{align}
% Additionally, $\A$ knows the secret key $k_i$ of $\PRF{i}$  of all the smart meters, thus can refine the submitted $\tilde{m_i}$s and obtain: 
% \begin{align}
%   \breve{m_i}  = \tilde{m_i}- \PRF{i} = m_i + s_i \hspace{5pt}  \forall i \in \Lcand
% \end{align}
% $\A$ also knows $MList$  that allows her to extract the masking values of all the non-challenged smart meters, i.e.
% \begin{align} \label{eq:si_view}
%     s_{i}= \breve{m_i} - m_{i,t} \mod k \hspace{5pt} \forall i \in \Lcand / \{SM_{i^*}, SM_{j^*}\}
% \end{align}
% So, it can further derive the sum of the challenged-smart meters masking values, i.e.
% \begin{align}
%  S_{i^*,j^*}= s_{i^*} +  s_{j^*} = S_N - \sum_{i \in \Lcand / \{SM_{i^*}, SM_{j^*}\}}  s_{i}
% \end{align}
% Therefore, the knowledge of $\A$ about the challenged smart meters come down to the sum of their randomnesses, i.e.  as well as their individual masked measurements, i.e. $S_{i^*,j^*}$ $\breve{m}_{i^*}$ and $\breve{m}_{j^*}$. The value of $S_{i^*,j^*}$ is independent of $b$ and thus provides no advantage for the adversary to win the game. In order to infer the value of $b$ from  $\breve{m}_{j^*}$ and $\breve{m}_{i^*}$, the adversary must be able to distinguish the measurements masked behind each of them. However, this should not be possible as long as the masking values $s_{i^*}$ and $ s_{j^*}$ are generated by a secure PRG whose output is indistinguishable from a random number generator. As such, the success of $\A$ is bound to the indistinguishability of the underlying PRG. If $\A$ can guess $b$ correctly and win the game, it implies that the underlying PRG is not cryptographically secure and  is distinguishable from a truly random number generator.
% \end{comment}
% %In the $\Unlink$ game, $\A$'s view to the challenged smart meters is limited to their sum of measurements, i.e. $s_{i^*} +  s_{j^*}$  as well as their individual masked measurements, i.e. $\tilde{m}_{i^*}$ and $\tilde{m}_{j^*}$. While the former is independent of $b$, the latter case can help the adversary to win the game if she manages to distinguish the measurements masked behind each of them. However, this should not be possible as long as the masking factors are generated by a cryptographically-secure PRG whose output is indistinguishable from a random number generator. As such, if $\A$ can guess $b$ correctly and win the game, it implies that the underlying PRG is not cryptographically secure.

% In the reduction proof, $B$ acts as the challenger for the unlinkability game and at the same time as the adversary for the PRG indistinguishability game. $B$ receives a vector of two values $\overrightarrow{S}=<s_0,s_1>$ which are either truly random or generated by a pseudo-random number generator. $B$ leverages the success probability of $\A$ to win the PRG game by using $s_0,s_1$ to mask the measurements of $SM_{i^*}$ and $SM_{j^*}$ (the challenged smart meters).
% %Let $U$ represent all non-challenged smart meters who are part of $\Lact$ i.e., $U=\{SM_i\in \Lact / \{SM_{i^{*}},SM_{j^{*}}\} \}$ and $U_{DC}$ represent the smart meters with an active link to $DC$ i.e., $U_{DC}=\{SM_i | (SM_i,DC) \in E'\} \}$.
% At the end of the game, $\A$'s view toward the challenged smart meters is limited to $S=s_0+s_1+\sum_{i \in \{SM_i\in \Lact / \{SM_{i^{*}},SM_{j^{*}}\} \}}$ and their individual masked measurements i.e., $\tilde{m}_{i^{*}}$,  $\tilde{m}_{j^{*}}$. %, and $\tilde{m}_{i}$  of $U_{DC}$. Due to the constraint imposed at step 3 of the game, the challenged smart meters must be able to contribute to the final aggregate i.e., they must be part of $\Lact$ and $U_{DC}$ and hence their masking values must be part of $S$, also their individual masked measurements must be given to $\A$. 
% The value of $S$ is independent of $b$ thus makes no help for the adversary. In order for the adversary to be able to make a correct guess, it needs to exploit $\tilde{m}_{i^{*}}$,  $\tilde{m}_{j^{*}}$. If $\overrightarrow{S}$ is truly random, then $\tilde{m}_{i^*}$ and $\tilde{m}_{j^*}$ look completely random to $\A$, which leaves $\A$ with no advantage to win the unlinkability game. In case  $\overrightarrow{S}$ is pseudo-randomly generated, $\A$ may have some advantage $\epsilon(1^{\lambda})$ to win the unlinkability game. % As illustrated in Equation \ref{eq:proof_masking_dc}, $B$ will win the PRG game if $\epsilon(1^{\lambda})$ (i.e., the advantage of $\A$ in breaking $\Unlink$) is non-negligible. $\square$
% Note that $\epsilon(1^{\lambda})$ tightly relates to the distinguishability of the PRG from truly random number generators. However, as the deployed PRG is secure, $\epsilon(1^{\lambda})$ is a negligible value which means the $\A$'s advantage in wining the unlinkability game is also negligible. As such, 
% if $\A$'s output $b'$ equals to $b$, then $B$ returns $0$ to the PRG challenger signifying that $ \overrightarrow{S}$ is pseudo-random, otherwise, outputs $1$ in the PRG game meaning $\overrightarrow{S}$ is truly random. $\square$
% % \begin{align} \label{eq:proof_masking_dc}
% %     & Pr [ B \text{ wins PRG game}] = \nonumber \\
% %     & |Pr[B \text{ outputs 0}| \overrightarrow{S} \text{ is R} ]-Pr[B \text{ outputs 0} | \overrightarrow{S} \text{ is PR}]| \nonumber  \\
% %     & |Pr[b==b' | \overrightarrow{S} \text{ is R}] - Pr[b==b' | \overrightarrow{S} \text{ is PR}]|  =  \nonumber \\
% %     & |\frac{1}{2} - \epsilon(1^{\lambda})|
% % \end{align}

% %=========================================
% % TODO uncomment for the full version
% %\input{proofs/PrivacyProofMaskingFull} 
% %=========================================
% \subsubsection{Proof of Theorem \ref{thm_masking}.(iii)}
% In order to prove that a collusion set is maximal, we show that any super set of the maximal set can launch a successful attack and break $\Unlink$. \\
% The collusion set (i) can only be extended by adding the $\DC$.  In the attack, we consider the worst case where adversary arranges the network in a way that the first active smart meter in the aggregation phase is $\SM_{i^*}$ and its next active link is $SM_{k}$. Since $SM_{k}$ gets $S_{i^*}=s_0+s_{i^*}$ and $\DC$ gets $\tilde{m_{i^*}}=m_{i^*}+s_{i^*}+\PRF{i^*}$ from $\SM_k$ they recover 
% $m_{i^*}=\tilde{m}_{i^*}-[S_{i^*}-s_{0}] -\PRF{i^*} \mod k$ and win the game. 
% %can only be extended by adding the $\DC$. In a successful attack, without loss of generality, we consider the adversary imposes the following arrangement: $\cdots SM_{i^*}\xrightarrow{} SM_k \cdots \xrightarrow{} SM_{j^*}$  where $SM_k$ is a the next active link of $SM_{i^*}$ and gets access to $S_{i^*}$. Together with $\DC$ knowing $\tilde{m_{i^*}}$ and $\tilde{m_{j^*}}$, they can derive $m_{i^*}$ through $ m_{i^*}= \tilde{m_{i^*}} - \PRF{i} - [S_{i^*} - s_0 - \sum_{i \in P} s_i]$ where $P$ is the set of contributing smart meters preceding $SM_{i^*}$.
% In collusion set (ii) we augment the adversarial set by adding  one smart meter namely $SM_{k}$. The adversary can break the privacy following the preceding attack scenario. 

% %In the attack, we consider the worst case where adversary arranges the network in a way that the first active smart meter in the aggregation phase is $\SM_{i^*}$ and its next active link is $SM_{k}$. Since $SM_{k}$ gets $S_{i^*}=s_0+s_{i^*}$ and $\DC$ gets $\tilde{m_{i^*}}=m_{i^*}+s_{i^*}+\PRF{i^*}$ from $\SM_k$ they recover $m_{i^*}=\tilde{m}_{i^*}-[S_{i^*}-s_{0}] -\PRF{i^*} \mod k$. 
% %\end{proof}
% % \begin{flushright}
% % $\square$ 
% % \end{flushright}
% %Thus, if $\epsilon(1^{\lambda})$ is non-negligible, the output of PRG is also distinguishable with non-negligible advantage of $\epsilon(1^{\lambda})$ and hence $B$ wins the underlying PRG game which contradicts with the initial ass%Initially, the challenger connects Note that due to the network model oracle, the adversary gets to decide on the contributing smart meters, in specific, the members of $L_{rem}$ and $L_{act}$. The challenger receives a vector of two values $<s_0,s_1>$ which are either truly random or generated by a pseudo-random number generator. The challenger uses these values to mask the measurements of $SM_{i^*}$ and $SM_{j^*}$ (the challenged smart meters at step 3 of the game). For the rest of the game, the challenger proceeds based on the protocol. Throughout this interaction, the  adversary gets to see the individual masked measurements i.e., $\tilde{m}_{i}$ as well as a the aggregate of masking values of a subset of smart meters as $S$. 

% \subsection{ Privacy Analysis of the Homomorphic  Aggregation Protocol}
% The following theorem \ref{thm_homo} states the privacy guarantee of the protocol based on homomorphic encryption which relies on the IND-CPA property. Essentially, the theorem states that the two maximal collusion sets are the ones described in Figure \ref{fig:privVisu2}.  

% % For this protocol, we consider two maximal collusion sets 1) $DC$ and 1) a subset of $N-2$ smart meters.
% % \subsubsection{Privacy Proof against $DC$}
% % In this adversarial setting, the adversary controls $DC$ whereas the challenger runs on behalf of all the smart meters. The privacy proof, as formulated in Theorem \ref{thm_masking_dc}, relies on the security of the underlying pseudo-random number generator. 
% \begin{theorem}[Privacy of the aggregation protocol using homomorphic encryption] \label{thm_homo}
% Consider the protocol of Figure \ref{fig: algoGeneralV02} with privacy-preserving computations done using homomorphic encryption as described in Section \ref{sec:improveFlow}. The followings hold where privacy is as defined in the $\Unlink$ game:
% \begin{itemize}
%     \item[(i)] If the underlying encryption scheme is CPA, the protocol provides privacy against an adversary consisting of $N-2$ colluding smart meters. 
%     \item[(ii)] The protocol provides information-theoretic privacy against the adversary controlling $\DC$. 
%  \item[(iii)] Both collusion sets above are maximal.
% \end{itemize}

% \end{theorem}


% %\input{tikz/privHomoOrig}
% \input{tikz/privHomoNew}



% \subsubsection{Proof of Theorem \ref{thm_homo}.(i)}
% In the reduction, $B$ acts as the challenger for the unlinkability game and as the adversary for the CPA game. $B$ gets the encryption public key $pk$ from the CPA challenger and hands it to the adversary. $\A$ outputs $m_0, m_1$, list $L$ and the network failure model $G'$ (note that $\A$ does not output $MList$ since the non-challenged smart meters are under its own control). Given $L$ and $G'$, $B$ checks that the challenged smart meters are part of $Lact$ and aborts if otherwise. 
% $B$ leverages the success power of $\A$  to win the CPA game by delegating the measurement assignment of challenged smart meters to the CPA challenger as explained next. $B$ crafts two message vectors $\overrightarrow{v_0}=(m_0,m_1)$ and $\overrightarrow{v_1}=(m_1,m_0)$ where each signifies an ordered assignment of $m_0$ and $m_1$ to $SM_{i^{*}}$ and $SM_{j^{*}}$, respectively. $B$ outputs $\overrightarrow{v_0}$ and $\overrightarrow{v_1}$ as part of the CPA challenge phase and obtains a cipher vector $\overrightarrow{C_b}=(c_b,c_{\hat{b}})$ where bit $b$ is selected randomly by CPA challenger. $B$ uses $c_b$ and $c_{\hat{b}}$ as the measurements of $SM_{i^*}$ and $SM_{j^*}$, respectively. The view of $\A$ in the game is one of the followings:
% 1)  $SM_{i^*}$ and $SM_{j^*}$ are each other's immediate neighbors in $\Lact$, in which case $\A$ as the non-challenged smart meters, obtain the aggregate of $SM_{i^*}$ and $SM_{j^*}$ encrypted measurements, i.e. $Enc_{pk}(m_b+m_{\hat{b}})$. 
% 2) Otherwise, $\A$, playing the immediate neighbors of challenged smart meters in $\Lact$, obtains the individual encrypted measurements of $SM_{i^*}$ and $SM_{j^*}$, i.e. $c_b=Enc_{pk}(m_b)$ $c_{\hat{b}}=Enc_{pk}(m_{\hat{b}})$. The former case does not carry any information about $b$ (since it is independent of $b$), whereas the latter case might lead to some leakage about $b$ if the deployed encryption scheme is not CPA-secure, i.e. if $\A$ can distinguish between the messages encapsulated in $c_{b}$ and $c_{\hat{b}}$ (i.e., to distinguish between  $\overrightarrow{v_0}$ and $\overrightarrow{v_1}$). $\A$ outputs its guess as $b'$, which $B$ sends directly to the CPA challenger. If $\A$ has non-negligible advantage to win the unlinkability game so does $B$ in the CPA-game. 


% %\input{proofs/PrivacyProofHomomorphicFull}

 


% \begin{comment}

% The algorithm contains two parts which aim at loosening the HBC assumption.
% First, note that we proved that the end of the round is determined by the smart meters and not by the $\DC$. While this makes no difference for an honest $\DC$, this limits the possibilities for a dishonest $\DC$: for example for masking the $\DC$ may try to send an $\EOR$ signal to the 2 neighboring smart meters of $\SM_i$, ($\SM_{i-1}$ and $\SM_{i+1}$) in order to get the final messages. From these messages $m_i$ can be simply computed from $m_i=\tilde{m_i}-(\SM_{i+1}-\SM_{i-1}$. An analogous method works for homomorphic encryption.\\
% Second, as already discussed in section \ref{sec:improveSecurity} the usage of the round-dependent PRFs prevents external eavesdroppers of the communication links from inferring useful information.
% \end{comment}

% % There are some protocols with higher privacy guarantees: there, nearly all smart meters could collude with $\DC$ (for example the low overhead protocol of Kursawe). However, in these protocols typically each pair of smart meters $i$ and $j$ share a common key $k_{ij}(t)$. One smart meter adds $k_{ij}(t)$ it to its measurement, the other one subtracts it so these shares sum up to zero. This pairwise addition and subtraction is done for all pairs. While this can be done effectively and has a higher privacy guarantee, it is not fault tolerant. If a single smart meter fails, the sum of shares do not cancel each other and the aggregate is useless.



% \subsubsection{Proof of Theorem \ref{thm_homo}.(ii)}
% The privacy proof against $DC$ is information-theoretic. This because the view of $\A$ toward the challenged smart meters is limited to their sum of measurements regardless of how adversary influences the network failure model $G'$ and the arrangement list $L$ (under any $G'$ and $L$, both challenged smart meters are guaranteed to be part of the aggregation due to step 3 of the $\Unlink$). $\A$ obtains the final aggregate  $A_t = m_b + m_{\hat{b}}+ \sum_{i \in \Lact/\{SM_{i^*},SM_{j^*}\}} m_{i,t}$  and can narrow it down to $m_b + m_{\hat{b}}$ by subtracting the measurements of non-challenged smart meters. However, the value of $m_b + m_{\hat{b}}$ is independent of $b$ thus conveys no information for breaking $\Unlink$ game. $\square$

% %as explained next. During the unlinkability game, the adversary decides on the exact measurements of the non-challenged smart meters, the measurements of challenged smart meters $m_0$ and  $m_{1}$ and  the network failure model $G'$ which influences the list $\Lact$ i.e., the contributing smart meters. The challenger randomly assigns $m_0$ and  $m_{1}$ to the challenged smart meters and at the end, $\A$ obtains the final aggregate  $A_t = m_b + m_{\hat{b}}+ \sum_{i \in \Lact/\{SM_{i^*},SM_{j^*}\}} m_{i,t}$ (recall that $\Lact$ embodies the challenged smart meters due to the checks done at step 3). $\A$ knows the measurements of the non-challenged smart meters i.e., $ \Lact/\{SM_{i^*},SM_{j^*}\}$, thus it can extract the aggregate of challenged smart meters' measurements from $A_t$ which is $A_t- \sum_{i \in \Lact/\{SM_{i^*},SM_{j^*}\}} m_{i,t}= m_b + m_{\hat{b}}$. However, the value of $m_b + m_{\hat{b}}$ is independent of choice $b$ and the adversary obtains no useful information from its interaction with the challenger to yield a correct guess $b'$.

% % \begin{align}
% %     A_t - \sum_{i \in \Lact/\{SM_{i^*},SM_{j^*}\}} m_{i,t}  & = \\
% %     \sum_{i \in \Lact} m_{i,t}- \sum_{i \in \Lact/\{SM_{i^*},SM_{j^*}\}} m_{i,t} & = \\
% %     \sum_{SM_{i^*},SM_{j^*}}m_{i,t} = m_b + m_{\hat{b}}
% % \end{align}

% \subsubsection{Proof of Theorem \ref{thm_homo}.(iii)}
% In order to prove that a collusion set is maximal, we show that any super set of the maximal set can launch a successful attack and break $\Unlink$.
% The collusion set (i) can only be extended by adding the $\DC$. In the attack, we consider the worst case where adversary arranges the network in a way that the first active smart meter in the aggregation phase is $\SM_{i^*}$ and its next active link is adversarial smart meter $SM_{k}$ which gets to see $S_{i^*}=E_{pk}(m_{i^*})$. Adversary also controls $\DC$ so has the decryption power and can retrieve $m_{i^*}= Dec(S_{i^*})$ and break the game.
% In collusion set (ii) the adversarial set by adding  one smart meter namely $SM_{k}$.  The adversary can break the privacy following the preceding attack scenario. 

% %\end{comment}
% $\square$


==> proofs/distinguisher.tex <==
\begin{figure*}
    \centering
		\begin{bbrenv}{A}
		
		% middle party
			\begin{bbrbox}[name=$B$, minheight=3.5cm]
			  \vspace*{1.1cm}
			    Choose $b$ uniformly from $\{0,1\}$\\
				$m_{i^*}=m_{b}+s_0, \ m_{j^*}=m_{\bar{b}}+s_1$\\ 
					 \vspace{0.2cm}\\
				 Set $b_{PRG}'=1$, \textbf{if} $b'=b$, \textbf{else} 0
		\end{bbrbox}
		
			
		% left
			\begin{bbrchallenger}{ChaU=AdvPRG}
				\begin{bbrbox}[name=$\A$, minheight=3.5cm]
				 %\vspace*{0.1cm}
				 Select $m_0, \ m_1$\\
				 \\ \\ \\
				run protocol\\
				Choose $b'$
				% $A_{\var{MI}}$ guesses, if $z \in D$\\
				% \textbf{if} \ $z \in D$ \ $b'':=1$ \ \textbf{else} \   $b'':=0$
				% 	\pseudocodeblock{
    %                 \pcif $z \in D$\\
    %                 \pcind \pcreturn $b'\leftarrow1$\\
    %                 \pcelse \pcreturn $b'\leftarrow0$\\}
				\end{bbrbox}
			\end{bbrchallenger}
		
		
	
		% right	
			\begin{bbroracle}{ChaPRG}
				\begin{bbrbox}[name=$\mathcal{C}_{PRG}$, minheight=3.5cm]
				    Choose $b_{PRG}$ uniformly from $\{0,1\}$\\
				    \textbf{if} $b_{PRG}=1$, \ $(s_0,s_1)\sim PRG$ \\ \textbf{if} $b_{PRG}=0$, \ $(s_0,s_1) \sim $ random
				    % \pseudocodeblock{
        %             \pcif $b=0$\ 
        %             \pcind $r \leftarrow M(\cali{D})$\\
        %             \pcelse $r \leftarrow M(\cali{D'})$\\}
                   \\ \\ \\ \\ 
                   \textbf{if} \ $b_{PRG}'= b_{PRG}$  %($\mathcal{A}_{PRG}$ wins) \ 
                   \textbf{return}  1, \textbf{else} 0
				    % \pseudocodeblock{
        %             \pcif $b'= b$\\
        %             \pcind \pcreturn $1$\\}
				\end{bbrbox}
			\end{bbroracle}
		
	
	
			

			
			\bbroracleqryfrom{top={$(s_0,s_1)$},beforeskip=4\baselineskip}
			\bbroracleqryto{top={$b_{PRG}'$},beforeskip=1.8\baselineskip}
			
			
			\bbrchallengerqryto{top={$m_0, \ m_1$}, beforeskip=2\baselineskip}
			\bbrchallengerqryfrom{top={$m_{i^*},m_{j^*}$}, beforeskip=2\baselineskip}
			\bbrchallengerqryto{top={$b'$}}%, beforeskip=\baselineskip}
		\end{bbrenv}    
		\caption{Construction of a PPT distinguisher to distinguish pseudorandom numbers from truly random ones, if one can break unlinkability}
    \label{fig:distinguisher}
\end{figure*}

==> proofs/distinguisherNew.tex <==
\begin{figure*}
    \centering
		\begin{bbrenv}{A}
		
		% middle party
			%\begin{bbrbox}[name=$B=\mathcal{C}=\mathcal{A}_{PRG}$, minheight=3.5cm]
			\begin{bbrbox}[name=$B$, minheight=4.9cm]
			  \vspace*{0.8cm}
			    Select $b \leftarrow \{0,1\}$\\
				$m_{i^*}=m_{b}+s_0, \ m_{j^*}=m_{\bar{b}}+s_1$\\ 
					 \vspace{0.2cm}\\
					 \\
				 \textbf{if} $b'=b$, set $b_{PRG}'=1$\\ \textbf{else} \hspace*{0.65cm} set $b_{PRG}'=0$
		\end{bbrbox}
				

 		% left	
			\begin{bbrchallenger}{ChaPRG}
				\begin{bbrbox}[name=$\mathcal{C}_{PRG}$, minheight=4cm]
				    Select $b_{PRG} \leftarrow \{0,1\}$\\
				    \textbf{if} $b_{PRG}=1$, \ $(s_0,s_1)\sim PRG$\\ 
				    \textbf{else} \qquad \qquad \ $(s_0,s_1) \sim $ random
				    % \pseudocodeblock{
        %             \pcif $b=0$\ 
        %             \pcind $r \leftarrow M(\cali{D})$\\
        %             \pcelse $r \leftarrow M(\cali{D'})$\\}
                  \\ \\ \\ \\ 
                  \\
                  \\
                  \textbf{if} \ $b_{PRG}'= b_{PRG}$ \textbf{return}  1\\
                  \textbf{else}  \hspace*{1.9cm} \textbf{return}  0
				    % \pseudocodeblock{
        %             \pcif $b'= b$\\
        %             \pcind \pcreturn $1$\\}
				\end{bbrbox}
			\end{bbrchallenger}
				

			
		% right
			\begin{bbroracle}{AdvPRG}
			\begin{bbrbox}[name=$\A$, minheight=4.9cm]
			\vspace*{0.1cm}
				 Select $m_0, \ m_1$\\
				\\	\\	 \\ \\ \\
				Choose $b'$
				\\
			\\
				% $A_{\var{MI}}$ guesses, if $z \in D$\\
				% \textbf{if} \ $z \in D$ \ $b'':=1$ \ \textbf{else} \   $b'':=0$
				% 	\pseudocodeblock{
    %                 \pcif $z \in D$\\
    %                 \pcind \pcreturn $b'\leftarrow1$\\
    %                 \pcelse \pcreturn $b'\leftarrow0$\\}
				\end{bbrbox}
			\end{bbroracle}
		

 			\bbrchallengerqryto{top={$(s_0,s_1)$},beforeskip=4\baselineskip}
 			\bbrchallengerqryfrom{top={$b_{PRG}'$},beforeskip=3.8\baselineskip}

			\bbroracleqryfrom{top={$(m_0, m_1)$}, beforeskip=2\baselineskip}
			\bbroracleqryto{top={$(m_{i^*},m_{j^*})$}, beforeskip=1.5\baselineskip}
			\bbroracleqryto{top={\papertitle},  edgestyle=<->}
			\bbroracleqryfrom{bottom={$b'$}, }%, beforeskip=\baselineskip}
			
			
		\end{bbrenv}    
		\caption{Construction of a PPT distinguisher $B$ which plays the unlinkability game as the challenger with the adversary $\A$ and which is the attacker of the indistinguishability game. If $\A$ wins the unlinkability game, $B$ can distinguish pseudorandom from random numbers. However, this is computationally hard.}
    \label{fig:distinguisher}
\end{figure*}

% \bbroracleqryfrom
% \bbroracleqryto
% \bbrchallengerqryto
% \bbrchallengerqryfrom

==> proofs/privacyDescriptionLong.tex <==
\textbf{Adversarial Model:}
Communication 
%channels 
links 
between smart meters and the $\DC$ are assumed to be secure and authenticated. Attackers are considered as honest-but-curious entities that follow the protocol but can collude and share their information to infer information about others. In addition, the adversary 
%is granted 
has 
the power to control the network failures, i.e., turn links off and on but not observe the messages. Link failures are considered bidirectional and their status does not change throughout the execution of \textit{one round} of the aggregation protocol. 
\begin{taggedblock}{long}
For aggregation used for monitoring purposes, the honest but curious assumption seems reasonable and is commonly employed in \cite{Li10b,Acs11a, Kursawe11a}. This is in contrast to the billing use case where the potential benefits of fraud leads to much less trust. Some papers aggregate also for billing and aim at fulfilling additional requirements such as verifiability of the bill or data integrity \cite{Borges15a, Fan14a, Ni17a}. This paper aims at improving the core of the aggregation method. Considering other orthogonal extensions may be future work. 
\end{taggedblock}

\textbf{Formally defining unlinkability of measurements:}
To formally capture the privacy objective under the designated adversarial model, we define the following privacy game, to be played between an adversary and a challenger, by adapting the smart meter’s data unlinkability game defined in \cite{Unterweger18b}.  The adversary controls all  colluding adversarial entities, whereas the challenger acts on behalf of the remaining honest parties.
The only restriction in this game is that at least two honest smart meters (out of $N$ total smart meters) are out of the adversary's control. These smart meters are called \textit{challenged smart meters}.
\begin{taggedblock}{medium}
Having less than two honest smart meters (i.e., only one honest) innately breaks the security objective, where the adversary can subtract the sum of $N-1$ known measurements from the final aggregate and extract the measurement of the remaining honest smart meter. Thus, no private aggregation protocol could satisfy such a definition with only one honest smart meter, under our adversarial model. However, even with assuming the existence of at least two honest smart meters, the adversary can pick two measurements to be assigned to the honest smart meters. 
\end{taggedblock}
\begin{taggedblock}{short}
The adversary picks two measurements to be randomly assigned to these two honest smart meters by the challenger. 
\end{taggedblock}
Thus, the adversary can even know the two measurements, but still cannot infer which measurement corresponds to which honest smart meter. The aggregation protocol preserves data unlinkability if the adversary cannot infer this assignment except with a probability \textit{negligibly} higher than a random guess. 

Our game extends the game of \cite{Unterweger18b}  with additional adversarial power as explained next:
\begin{itemize}
 \item 
\begin{taggedblock}{short}
   In step 2 of the extended game, the adversary additionally knows the individual measurements of any subset of the $N-2$  \textit{non-challenged} smart meters (in addition to the two challenged smart meters). This additional power models a scenario where that knowledge might get exposed to the adversary indirectly, without the households' intention. Note that this does not include the secret shares or ciphertexts, which are only known for the \textit{colluding} smart meters that are under his control.
\end{taggedblock}
\begin{taggedblock}{medium, long}
    The adversary additionally knows the individual measurements of any subset of the $N-2$ smart meters (in addition to the two challenged smart meters). This additional power models the real-life scenario where the adversary may have background knowledge about the electricity consumption of some of the households participating in the aggregation protocol (e.g., due to being neighbors). 
    That knowledge might get exposed to the adversary indirectly, without the households' intention.
    In the extended game, we therefore consider the worst-case scenario where the adversary manages to learn the measurements of all the \textit{non-challenged} smart meters as side-knowledge. Note that this does not include the secret shares or ciphertexts, which are only known for the \textit{colluding} smart meters. In the game, this is modeled by allowing the adversary to specify the individual measurements of $N-2$ non-challenged smart meters in step 2.
\end{taggedblock}
 \item
\begin{taggedblock}{short}
    The adversary is additionally allowed to cut off communication lines, i.e., to change the status of network links from on to off. This could happen during a network attack even without touching smart meters. While this attack is likely having a different goal, privacy will be preserved as long as the two challenged smart meters remain contributing.
    The adversary specifies the network failures by outputting a sub-graph $G'=(V', E')$ of $G$ with the same parties $V'=V$ but only a subset of working links $E'\subseteq E$.
Throughout the game, messages can only be exchanged between two entities $V_i$ and $V_j$ when the connecting edge is in $E'$ (i.e., when $(V_i,V_j) \in E'$, solid lines in Figure \ref{fig:exNetwork0}). Otherwise, the link is off (dashed lines) and no data transmission can take place.
\end{taggedblock}
\begin{taggedblock}{medium, long}
     The adversary dictates the network failure model, i.e., the status of network links being on or off, provided that the challenged smart meters will remain contributing. %This condition is modeled by having the challenger check that restriction resulting in a losing adversary in case of not passing the check. 
    To enable this, the network is modeled as an undirected graph $G=(V, E)$ in which $V$ is the set of vertices corresponding to the entities involved in the aggregation protocol (e.g., smart meters and $\DC$) and $E$ is the set of edges corresponding to the presence of a network link between the two connected vertices.  The adversary signifies the network failure model by outputting a sub-graph $G'=(V', E')$ of $G$ where $G'$ has an identical set of vertices (i.e., $V=V'$), but contains a subset of edges (i.e., $E'\subseteq E$).  $E'$ represents the set of network links that are working and $E \setminus E'$ indicates the offline links. Messages can be exchanged between two entities only if there is an edge connecting those entities in $E'$. Throughout the game, when a message exchange between $SM_i$ and $SM_j$ is required, the challenger checks for an edge connecting $SM_i$ and $SM_j$ in $E'$ (i.e., whether $(SM_i,SM_j) \in E'$). Upon the existence of such an edge, a message transmission takes place; otherwise, the link is down and the challenger skips the data transmission. 

In the scenario exemplified in Figure \ref{fig:exNetwork0}, the nodes of both the network graph $G$ and the network failure graph $G'$ consists of all the parties. However, while $E$ consists of all (solid and dashed) links, only the solid ones appear in $E'$; the dashed links denote the failing links in $E'\setminus E$.
\end{taggedblock}

\end{itemize}  
% \def\xDC{4}
% \def\yscale{0.8}
% \def\bend{50}
% \def\bendz{15}

% \begin{figure}[htb]
% 	\centering
% 	%\input{tikz/G.tikz}
% \caption{The network graph $G$ corresponding to Figure \ref{fig:exNetwork0}.}
% \label{fig:G}

% \end{figure}
% \begin{figure}[htb]
% 	\centering
% 	%\input{tikz/tikzNetwork2.tikz}
% \caption{The network failure graph $G'$ corresponding to Figure \ref{fig:exNetwork0}.}
% \label{fig:GPrime}
% \end{figure}

The formal definition follows. 


==> proofs/proofPrivacyHomoShort.tex <==
\begin{proof}
(iii) Case (i) is the same as for to the masking case, in case (ii) $\DC$ uses $S_1$ from $\SM_2$ to calculate $D_{sk}(S_1/S_0)=m_2$.
\end{proof}

==> resilience.tex <==
% sparse certificates for k-connectivity: https://en.wikipedia.org/wiki/K-connectivity_certificate https://link.springer.com/article/10.1007%2FBF01758778
In the termination theorem error-resilience is described in the following way:   the aggregate can be calculated despite non-working smart meters or communication channels, if at least $\nmin$ smart meters will be active. No additional round is needed. 
While this error-resilience guarantee is a good first step it has the drawback that it is rather implicit: according to the guarantee it is important to have enough active smart meters. A natural next step is to consider of how to change the setting such that the number of active smart meters is maximized.

The number of active smart meters is determined implicitly by (a) the initial ordering of the smart meters and b) the places where errors occur. These two factors determine the path along the smart meters. While one can not influence the occurrence of the errors, the initial ordering of the smart meters can be changed. 

So far the ordering of the smart meters was already determined by the $\DC$. Since there is no justification for this ordering it is the first thing that can be easily changed. If one removes the ordering and defines the sending list as an unordered set the way the information should flow is not clear at all. The situation lends itself for being formulated using graphs: the smart meters and the $\DC$ are modeled as nodes and the pairwise connection are modeled as undirected edges. For the calculation of $S$ one needs to solve the following graph theoretic problem: Find a path (preferably a cycle) in this graph that starts at $\DC$, visits as many smart meters as possible but at least $\nmin$ of them and then ends at $\DC$. Note that for both masking and homomorphic encryption for the sake of privacy there is a necessary condition that the $\DC$ only acts at the beginning and the end when shares are summed and ciphertexts are multiplied, respectively. 
While this kind of problem may look rather familiar, in the given case the graph is not not known beforehand since the edges or nodes that fail in a round are not known in advance. 

Note, that in  algorithm \ref{fig: algoGeneralV02} some information is already got in the first step, where the smart meters send their masked values to the $\DC$. From this, a) the working smart meters at the round and b) the working links to the $\DC$ can be inferred. Due to this reduction of uncertainty the algorithm gains its simplicity. 

Checking the graph theory literature, several useful concepts can be found. 
%Due to the simplification node failures are ruled out. 
In the design phase of the ordering k-edge connectivity which is already very well studied \textbf{cite Parter} would ensure that the graph remains connected, if the graph stays connected despite the removal of k-1 edges (links). Consider as an example the network in Figure \ref{fig:exNetwork0}. The subgraph induced by the smart meters is 2-connected. It is at most 2-connected because the minimum degree of a node is 2, it is also not 1-connected, because it contains no bridge. Since the more complicated improved algorithm uses this graph, it yields an aggregate of all the smart meters even if one arbitrary link between smart meter fails. In contrast, the simplified algorithm only considers the subgraph induced by the nodes with a connection to the $\DC$ (nodes 1, 2 and 5). This subgraph is only a straight line between smart meters, so any failure of a single link between these nodes leads to the effect that not all smart meters will contribute to the aggregate. More concretely, the failure of the link between smart meters 3 and 5 would yield to an aggregate of only smart meters 1 and 2 for the simplified algorithm while the complicated algorithm gets an aggregate of all 3 smart meters without using the link in this example.

While k-connectivity is useful and guarantees that a path connecting all nodes exist this is not exactly the problem at hand. On one hand our graph-theoretic problem is simpler since not \emph{all} the nodes need to contribute to the sum, only at least $\nmin$. On the other hand it is harder because it still stays open, how such a path can be found, since the existing edges are not known.

Another way to improve the resilience would be to monitor the failures and re-design the sending list according to the failure statistics. This section should be understood as a starting point of future research. Good methods may be developed by specialists in the design of robust communication networks or specialists from graph theory.

% Apart from considering robustness due to failures one could also try completely different ways to find a path. For example, a smart meter could try to contact a random smart meter from the remaining, unvisited smart meters $\Lcand$. In case there is no connection, it could try a number of other remaining smart meters. If enough smart meters have already contributed it could also decide to send $S$ to the $\DC$. If not, it could try to send it back to the smart meter from which it was contacted. This raises the question how likely it is, that enough meters contribute to the aggregate.
% As a result, the presented algorithm is only advisable, if a high fraction $p$ of the links exist, since only then it yields an aggregate consisting if at least $\nmin$ measurements. The algorithm, however, could be modified in order to alleviate this problem. For example, one does not have to immediately remove a smart meter from $\Lcand$. With additional bookkeeping one could do this for example after the third unsuccessful attempt to contact it. This is just meant as an example how removing the ordering of the smart meters could also lead to different kinds of failure-tolerant algorithms. In this view, this paper may serve as a starting point for further research in that direction.



% \subsection{Discussion and Other Variants}

% The algorithm can be explained by means of an illustrative toy example network shown in Figure \ref{fig:exNetwork2} with $\nmin$ set to 3. At the beginning all smart meters except smart meter 4 will send their masked value to the $\DC$. Thus, $\Lcand=\{1,2,3,5,6\}$ and $\SM_4$ will not occur in the algorithm any more. This makes sense, because it can not send its masked measurement to the $\DC$ during this round. 

% If $\DC$ would initially select $i=3$, $\SM_3$ would get active, so it would set $\Lact=\{3\}$ and $\Lcand=\{1,2,5,6\}$. After updating $S$, $\SM_3$ would not be able to contact any other smart meter (note that there is a link to $\SM_4$, but $\SM_4$ can not be selected since it is not in $\Lcand$). Therefore the round would end without an aggregate since $\vert \Lact \vert =1<\nmin$.

% If $\DC$ would initially select $i=1$, $\SM_1$ would get active. The algorithm could only continue further if $\SM_1$ would randomly select $\SM_2$ as next party in the algorithm. If this would be the case, all 4 smart meters would contribute to the aggregate since all remaining links work in this round. As another example, three smart meters would only contribute to the aggregate in cases of $(5,2,1)$ or $(6,2,1)$. Note that the order of selection is important.

% This raises the question how likely it is, that enough meters contribute to the aggregate. 
% The probability depends on $\nmin$, the number of smart meters that can connect to the $\DC$ and the number of links between smart meters. The example shown in Figure \ref{fig:exNetwork2} may seem too pessimistic, since out of the $\frac{n(n-1)}{2}=15$ links between the 6 smart meters, only 7 work. In order to reach $\nmin=3$, the first 2 selected links would need to exist. Assuming that a proportion $p\in [0,1]$ links randomly exist between all pairs of smart meters that already have established a connection to the $\DC$, the probability to have at least 3 smart meters contributing is roughly $p^{\nmin-1}=p^2$. Note that $p$ only depends on the connections of working smart meters, since if a smart meter does not work, it could not have sent its masked value to the $\DC$ at the beginning of the round.



% The routing could of course be improved by analyzing different rounds and maybe collecting statistics about which links are working or not. If one has some knowledge or reasoning about that one could order the smart meters such that subsequent smart meters likely have a connection. Then the original algorithm from \cite{Knirsch16a} would be a very good choice, maybe with a modification to send the masked values at the beginning of a round.

% For both the algorithm in \cite{Knirsch16a} and the one presented here the routing is   primarily controlled by smart meters. If one assumes Honest But Curious (HBC) parties, one could also give more control over the routing to the $\DC$ which could try to establish a connection graph and use algorithms from graph theory to optimize routing. While these kind of optimizations are interesting by themselves, they are not the topic of this paper. However, it should be noted that routing control has a consequence on privacy in the case of collusions. As shown later, in the worst case only the predecessor and the successor of a smart meter need to collude with the $\DC$ for revealing its measurement. Therefore, giving routing control to the $\DC$ would make it easier for him to collude with the right two parties. This is one reason why giving more control to smart meters is favored in this paper. Note that the subsequent privacy analysis that assumes HBC parties that may collude does not distinguish between these two main variants, because it always considers the worst case scenario that satisfies the given assumptions.




==> tikz/algoGeneralV01.tex <==
\begin{algorithm}[h!]
	%\setstretch{0.8}
	\vspace{1mm}
	    \tcc{Sending of initial data:}
		All $\SM_i$ send $\langle t,i,\mathrm{data}_i\rangle$ to $\DC$\\
		$\DC$ sets $\Lcand=( i\vert \ \mathrm{data}_i$ was received$)$\\
		\textbf{If} ($\vert \Lcand \vert \geq \nmin$): stop round $t$.\\ 
		$\DC$ sets $\Lact=\{\}$\\
		$\DC$ sets or calculates $S$\\
		\tcc{Start of aggregation}
		$\DC$ chooses first entry $i$ from $\Lcand$\\
		$\DC$ sends $\langle S, \ \Lcand, \ \Lact\rangle$ to  $\SM_i$\\
		\tcc{$\SM_i$ takes over}
		$\SM_i$ sends $\Ackring$ back\\
		$\SM_i$ calculates $S_{i}$ from $S$ and sets $S=S_i$\\
		$\SM_i$ sets $\Lact=\Lact \cup \{i\}, \ \Lcand=\Lcand \setminus \{i\}$\\
		
		
		
		\eIf{$(\Lcand \neq \{ \}) \ \&  \ (\vert \Lcand \cup \Lact \vert \geq \nmin)$}
    		{
		    $\SM_i$ chooses next $j\in \Lcand$\\
		    $\SM_i$ sends $\langle S, \ \Lcand, \ \Lact\rangle$ to  $\SM_j$\\  
		    \If{\rm{no} $\Ackring$ from $\SM_j$}
		        {
		        $\SM_i$ sets $\Lcand=\Lcand \setminus \{j\}$\\
		        \eIf{$\Lcand = \{ \}$}{sendFinalMessage}{try next $\SM_j$}
		        }
		    }
    		{
    		sendFinalMessage
    		}

% 		$\SM_i$ randomly chooses next $j\in \Lcand$\\
% 		$\SM_i$ sends $\langle S, \ \Lcand, \ \Lact\rangle$ to  $\SM_j$\\
% 		\While{ (\rm{no} $\Ackring$ from $\SM_j$) \& ($\vert \Lcand \cup \Lact \vert \geq \nmin$)}
% 		{
% 		$\SM_i$ sets $\Lcand=\Lcand \setminus \{j\}$ and tries next $\SM_j$
% 		}
% 		\eIf{$\vert \Lcand \cup \Lact \vert \geq \nmin$}
% 		{
%     		\eIf{ \rm{successful (i.e.} $\Lact \neq \{ \}$)}
%     		{idle}
%     		{send $\langle \EOR, \ S, \ \Lact \rangle$ to $\DC$}
% 		}
% 		{
% 		send $\langle \EOR \rangle$ to $\DC$
% 		}

		\tcc{Finish the round at $\DC$:}
		\If{$\DC \ \mathrm{receives} \ \langle \EOR, \ S, \ \Lact  \rangle$}
		{
		$\DC$ \rm{does some final calculations with} $S$
	    }
	\caption{Generalized algorithm, version 1}  \label{fig: algoGeneralV01}
\end{algorithm}

==> tikz/algoIntermediate.tex <==
\begin{algorithm}[ht!]
	\setstretch{0.8}
	\vspace{1mm}
	\textbf{Initialization}\\
	%$\DC$ provides a sending list $\Lfull$ to all smart meters\\
	$\DC$ shares a key $k_i$ with each smart meter $\SM_i$\\
	\vspace{-2mm}
	\hrulefill \\
	\For{\rm{each round} $t \leq T$}
	{
		
% 		\textbf{One round of reading }$t$\\
% 		Start with the $\DC$: $h=0, SM_0=\DC$, $\SM_i=\SM_1$\\
% 		$\DC$ picks random $s_0$ and sets $S=s_0$\\
% 		\While{$\Ackring$ \rm{not received from} $\SM_i$}
% 		{
% 			i=i+1\\
% 			send $\langle \Lfull,t,\Lact=\{\}\rangle$ to next $\SM_i$\\
% 		}
% 		\eIf{$i \leq N-\nmin$}
% 		{
% 		$\DC$ sends $\langle S \rangle$ to $\SM_i$
% 		}
% 		{
% 		Algorithm stops
% 		}
		
		$\DC$ picks random $s_0$, sets $S=s_0$, $i=1$\\
		$\DC$ sends $\langle t,\Lfull,\Lact=\{\}\rangle$ to $\SM_i$\\
		\eIf{$\Ackring$ \rm{received from} $\SM_i$ }
		{
		$\DC$ sends $\langle t, S \rangle$ to $\SM_i$ 
		}
		{
		\eIf{$i < N-\nmin$}
		{
		contact next $\SM$ as above: $i=i+1$
		} 
		{
		Stop round $t$ (not enough measurements)
		}
		}
		
		\tcc{$\SM_i$ takes over:}
		\If{$\langle t,\Lfull,\Lact \rangle$ \rm{received from previous} $\SM$}{
			$\SM_i$ sends $\Ackring$ back to $\SM$}
		\If{$\langle t,S \rangle$ \rm{received from previous} $\SM$}
		    {
			$\SM_i$ picks random $s_i$ and sets $\tilde{m}_{i}= m_{i,t}+s_{i} + \PRFj \mod k$\\
			$\SM_i$ sends $t,\tilde{m}_{i}$ to $\DC$
			}
		\If{$\DC$ \rm{gets} $t,\tilde{m}_{i}$ \rm{from} $\SM_i$}
			{
			$\DC$ stores $\tilde{m}_{i}$\\
			$\DC$ sends $\Ackm$ to $\SM_i$
			}
			
		\If{$\Ackm$ \rm{received from} $\DC$}
		    {
			$\SM_i$ sets $S_{i}= S+s_{i} + \PRFj \mod k$\\
			$\SM_i$ sets $\Lact=\Lact \cup \{i\}$\\
    % 			\If{$\vert \Lact \vert \geq \nmin$}
    % 			{
    % 				send $\mathrm{L}_i:=\Lact$ to $\DC$\\
    % 				$\DC$ stores $L_i$
    % 			}
		    }
    		\While{$\Ackring$ \rm{not received from next in }$\Lfull$}
    		{
    			send $\langle t,\Lfull,\Lact \rangle$ to next in $\Lfull$
    		}
    		\If{\rm{next reached party is a }$\SM$}
    		{$\SM_i$ \rm{sends} $\langle t,S \rangle$ \rm{forward to} $\SM$}
    		\tcc{Check for End of Round $t$}
    		
    		\If{\rm{next reached party is }$\DC$}
    		{
    		    \eIf{$\vert \Lact \vert \geq \nmin$}
    		    {$\SM_i$ \rm{sends} $\langle t,\EOR,\Lact,S_i  \rangle$ \rm{to} $\DC$}
    		    {$\SM_i$ \rm{sends} $\langle t, \EOR \rangle$ \rm{to} $\DC$}
    		}
    		\If{\rm{no party is reached}}
    		{$\SM_i$ sends $\langle t,\EOR \rangle$ back to activating $\SM$}
    		\If{$\SM_i$ \rm{receives} $\langle t,\EOR\rangle$}
    		{
    		\eIf{$\SM_i\in \Lact$}
    		    {$\SM_i$ sends $\langle t,\EOR,\Lact, S_i \rangle$ to $\DC$}
    		    {$\SM_i$ sends $\langle t,\EOR \rangle$ to its activating $\SM$}
			}	
		\tcc{Finish the round at $\DC$:}
		\If{$\DC \ \mathrm{receives} \ \langle t,\EOR,\Lact, S_i \rangle$}
		{
		
		
% 		\While{\rm{waiting for round} $t$ \rm{to finish}}
% 		{
% %			\If{$L_i$ \rm{is received from} $\SM_i$}
% %			{store $L_i$}
% %			\If{\rm{round} $t$ \rm{finishes}}
% 			{
% 				pick $\mathrm{best} = \argmax_{i}\vert L_i \vert$\\
% 				send $\AckL$ to $\SM_{\mathrm{best}}$\\
% 				\If{$\SM_{\mathrm{best}}$ \rm{receives} $\AckL$ \rm{from} $\DC$}{Send $\langle S_{\mathrm{best}} \rangle$ to $\DC$}
				
				$\DC$ \rm{calculates the Average} $A_t = \left[\sum\limits_{i \in L_{\mathrm{best}}} \tilde{m}_{i} - \PRFj \right]- S_i$
		}
	}
	\caption{Improved algorithm}  \label{fig: algonew}
\end{algorithm}

==> tikz/algoSimple.tex <==
% old version of the simple algorithm

\begin{algorithm}[h!]
	\setstretch{0.8}
	\vspace{1mm}
	    \tcc{Sending of masked messages:}
	    All $\SM_i$ pick random $s_i\in \mathbb{Z}_k$ and set $\tilde{m}_{i}= m_{i,t}+s_{i} + \PRFj \mod k$\\
		All $\SM_i$ send $\langle t,i,\tilde{m}_{i}\rangle$ to $\DC$\\
		$\DC$ sets $\Lcand=( i\vert \ \tilde{m}_{i}$ was received$)$\\
		\textbf{If} ($\vert \Lcand \vert \geq \nmin$): stop round $t$.\\ 
		$\DC$ sets $\Lact=\{\}$\\
		$\DC$ chooses random $s_0\in \mathbb{Z}_k$ and sets $S=s_0$\\
		\tcc{Start of aggregating the shares}
		$\DC$ chooses first entry $i$ from $\Lcand$\\
		$\DC$ sends $\langle S, \ \Lcand, \ \Lact\rangle$ to  $\SM_i$\\
		\tcc{$\SM_i$ takes over}
		$\SM_i$ sends $\Ackring$ back\\
		$\SM_i$ calculates $S_{i}= S+s_{i} \mod k$\\
		$\SM_i$ sets $S=S_i, \ \Lact=\Lact \cup \{i\}, \ \Lcand=\Lcand \setminus \{i\}$\\
		$\SM_i$ randomly chooses next $j\in \Lcand$\\
		$\SM_i$ sends $\langle S, \ \Lcand, \ \Lact\rangle$ to  $\SM_j$\\
		\While{ (\rm{no} $\Ackring$ from $\SM_j$) \& ($\vert \Lcand \cup \Lact \vert \geq \nmin$)}
		{
		$\SM_i$ sets $\Lcand=\Lcand \setminus \{j\}$ and tries next $\SM_j$
		}
		\eIf{$\vert \Lcand \cup \Lact \vert \geq \nmin$}
		{
    		\eIf{ \rm{successful (i.e.} $\Lact \neq \{ \}$)}
    		{idle}
    		{send $\langle \EOR, \ S, \ \Lact \rangle$ to $\DC$}
		}
		{
		send $\langle \EOR \rangle$ to $\DC$
		}
		\tcc{Finish the round at $\DC$:}
		\If{$\DC \ \mathrm{receives} \ \langle \EOR, \ S, \ \Lact  \rangle$}
		{

		$\DC$ \rm{calculates the Average} $A_t = -S-s_0+\sum\limits_{i \in \Lact} \tilde{m}_{i} - \sum\limits_{i \in \Lact} \PRFj$
	}
	\caption{Final, simplified algorithm}  \label{fig: algoSimple}
\end{algorithm}

==> tikz/oldAlgoNew.tex <==
%\begin{algorithm}[h!]
%\setstretch{0.8}
%\vspace{1mm}
%\textbf{Initialization}\\
%%$\DC$ provides a sending list $\Lfull$ to all smart meters\\
%$\DC$ shares a key $k_i$ with each smart meter $\SM_i$\\
%\vspace{-2mm}
%\hrulefill \\
%\For{\rm{each round} $t \leq T$}{
%\textbf{One round of reading }$t$\\
%Start with the $\DC$: $i=0$, $\SM_i=\DC$\\
% $\DC$ picks random $s_0$ and sets $S=s_0$\\
%\While{$\Ackring$ \rm{not received from next} $\SM_j$}{
%	send $\langle \Lfull,t,\Lact=\{\}\rangle$ to next $\SM_j$
%}
%$\DC$ sends $\langle S \rangle$ forward to $\SM_j$\\
%\tcc{$\SM_j$ takes over:}
%Receiving $\SM_j$ sends $\Ackring$ back to $\SM_i$\\
%$\SM_i$ sends $\langle S \rangle$ forward to $\SM_j$\\
%$\SM_j$ picks random $s_j$ and sets $\tilde{m}_{j}= m_{j,t}+s_{j} + \PRFj \mod k$\\
%$\SM_j$ sends $\tilde{m}_{j}$ to $\DC$\\
%$\DC$ stores $\tilde{m}_{j}$\\
%$\DC$ sends $\Ackm$ to $\SM_j$\\
%\If{$\Ackm$ \rm{received from} $\DC$}{
%	$\SM_j$ sets $S_{j}= S+s_{j} + \PRFj \mod k$\\
%	$\SM_j$ sets $\Lact=\Lact \cup \{i\}$\\
%}
%\If{$\vert \Lact \vert \geq \nmin$}
%{
%	send $\mathrm{L}_j:=\Lact$ to $\DC$\\
%	%$\DC$ sends $\AckL$ to $\SM_j$\\
%	\If{$\AckL$ \rm{received from} $\DC$}{Send $\langle S_{\mathrm{best}}:=S_j \rangle$ to $\DC$}
%}
%\While{$\Ackring$ \rm{not received from next} $\SM_i$}{
%	send $\langle \Lfull,t,\Lact \rangle$ to next $\SM_i$
%}
%\tcc{Finish the round at $\DC$:}
%\While{\rm{waiting for round} $t$ \rm{to finish}}
%{
%\If{$L_j$ \rm{is received from} $\SM_j$}
%{store $L_j$}
%\If{\rm{round} $t$ \rm{finishes}}
%{
%	pick $\mathrm{best} = \argmax_{j}\vert L_j \vert$\\
%	send $\AckL$ to $\SM_{\mathrm{best}}$\\
%	Calculate Average $A_t = \left[\sum\limits_{j \in L_{\mathrm{best}}} \tilde{m}_{j} - \PRFj \right]- S_{\mathrm{best}}$
%}
%}
%}
%\caption{Improved aggregation algorithm}  \label{fig: algonew}
%\end{algorithm}


==> tikz/privGuarantee.tex <==
   \begin{collusiontable}
    \entityname{Alice}
    \entityname{Bob}
    \entityname{C.}
    \nomoreentitynames

    \collusion{heuristic}
    \collusion[0.8]{hard} \collusioncomment[white]{left}{*}
    \collusion{heuristic}
    \nextcollusionset
    
    \collusion{informationtheoretic}
    \collusion{insecure}
    \collusion[0.5]{informationtheoretic}
    \nextcollusionset
   \end{collusiontable}

%   \begin{minipage}{0.6\textwidth}
%     \begin{tabular}{ll}
%       \textbf{Improved Masking Protocol} & %
%       \begin{collusiontable}[baseline=(current bounding box.base)]
%         \entityname{$\SM\ {\scriptstyle 1..N}$}
%         \entityname{$\DC$}
%         \nomoreentitynames

%         \collusion[0.95]{informationtheoretic} \collusioncomment[white]{left}{\tiny $N-1$}
%         \collusion{insecure}
%         \nextcollusionset

%         \collusion{insecure}
%         \collusion{hard}
%         \nextcollusionset
%       \end{collusiontable}
%     \end{tabular}
%   \end{minipage}
%   \hfill
%   \begin{minipage}{0.35\textwidth}
%     \centering
%     \printcolorkey[baseline=(current bounding box.base)]
%   \end{minipage}
%   \caption{Privacy visualization for the presented improved masking protocol: The row color indicates the privacy level achievable when all colored entities of the row collude, e.g., $N-2$ smart meters and the data concentrator (first row in the first panel). Columns indicate entities and colors privacy levels as illustrated in the legend.}
%   \label{fig:privacy-visualization}


==> tikz/privHomoOrig.tex <==
\begin{figure}[htb]
    \centering
    \begin{minipage}{0.3\textwidth}
    %\begin{tabular}{ll}
    
      \begin{collusiontable}[baseline=(current bounding box.base)]
        \entityname{$\SM\ {\scriptstyle 1..N}$}
        \entityname{$\DC$}
        \nomoreentitynames

        \collusion[0.95]{hard}
        \collusioncomment[white]{left}{\tiny $N-1$}
        \collusion{insecure}
        \nextcollusionset

        \collusion{insecure}
        \collusion{hard}
        \nextcollusionset
      \end{collusiontable}
      
    %\end{tabular}
    \end{minipage}
          \hfill
          %\hspace{0.1cm}
  \begin{minipage}{0.12\textwidth}
    \centering
    \printcolorkey[baseline=(current bounding box.base)]
  \end{minipage}
        
    \caption{Privacy guarantee when homomorphic encryption is employed.}
    \label{fig:privVisu2}
\end{figure}

==> tikz/privMaskingOrig.tex <==
\begin{figure}[htb]
    \centering
    \begin{minipage}{0.3\textwidth}
    %\begin{tabular}{ll}
    
      \begin{collusiontable}[baseline=(current bounding box.base)]
        \entityname{$\SM\ {\scriptstyle 1..N}$}
        \entityname{$\DC$}
        \nomoreentitynames

        \collusion[0.95]{informationtheoretic} \collusioncomment[white]{left}{\tiny $N-1$}
        \collusion{insecure}
        \nextcollusionset

        \collusion{insecure}
        \collusion{hard}
        \nextcollusionset
      \end{collusiontable}
      
    %\end{tabular}
    \end{minipage}
          \hfill
          %\hspace{0.1cm}
  \begin{minipage}{0.12\textwidth}
    \centering
    \printcolorkey[baseline=(current bounding box.base)]
  \end{minipage}
        
    \caption{Visualization of privacy guarantee when masking is used as a privacy-preserving method (visualized using the tool developed in \cite{Unterweger18b})}
    \label{fig:privVisu1}
\end{figure}
 

==> variousLengths/existingAlgosShort.tex <==
Aggregation protocols aim at privately  summing the values of a given set of smart meters. The main methods (sometimes combined) are: masking \cite{ Kursawe11a, Erkin12b, Acs11a, Marmol13a, Knirsch16a, Bonawitz17a}, additive homomorphic encryption \cite{Shi11a, Engel17a, Li10a, Chan12a, Rastogi10a, Erkin12b},
%,ElGamal85a,Cramer97a} 
and  multiparty computation with secure secret sharing \cite{Danezis13a, Bonawitz17a, Mustafa19a}. 
%and multi-resolution methods aim at providing different resolutions to different parties. 
%%The focus of this paper lies on improving the underlying aggregation method with respect to failures, i.e. non-working smart meters or communication links. 
%For privacy reasons the protocol should be mostly performed by the smart meters themselves, in addition we only include the $\DC$ in order to not being dependent on lack of collusions between additional parties. 
%differential privacy is not considered further. 

% Since smart meters are limited in terms of calculation performance we want to avoid costly asymmetric cryptographic methods and therefore rule out methods that use homomorphic encryption like Li \cite{Li10a}, Borges IKUP \cite{Borges14a}, Erkin \cite{Erkin12a}, Erkin CRT \cite{Erkin15b}, Engel \cite{Engel13e}, Rane \cite{Rane15a}, Chan \cite{Chan12a}, Rastogi \cite{Rastogi10a} and Shi \cite{Shi11a}. 
%%As already stated in \cite{Knirsch16a},
Many papers propose privacy-preserving protocols  without providing a mechanism that works in case of faulty smart meters or non-working communication links \cite{Shi11a, Kursawe11a, Engel17a, Danezis13a}. Only a small number of papers discuss fault-tolerance (typically only failures of smart meters but not communication links).
%However, it may also be the case that the smart meter still works, but the communication between smart meters fail.
In \cite{Li10a}, aggregation using homomorphic encryption 
proceeds along an aggregation tree. A failing node would result in loss of values for all meters of the subtree rooted at that node.
%an additional aggregation along the tree, moreover values are lost also for all its children. 
In \cite{Chan12a} this problem is solved and the solution can  also be applied to the methods of \cite{Shi11a} and \cite{Rastogi10a}. 
However, to cover all functioning nodes, each node would need to perform roughly $\lfloor \log_2(n) \rfloor +1$ costly homomorphic encryption operations. This computational overhead for devices with low computational power, such as smart meters, should be avoided. 
The protocol of \cite{Erkin12b} combines homomorphic encryption with masking in the exponent of Paillier's encryption scheme \cite{Paillier99a}. In case of malfunctioning smart meters, missing random numbers are proposed to be retrieved by additionally contacting a trusted third party (the manufacturer) that can provide the missing information in a privacy-preserving way.

In \cite{Acs11a}, masking is employed with pairwise random shares that cancel each other in clusters of smart meters. Since missing shares would destroy the result, the corresponding counterparts need to be queried in an additional round.
In \cite{Marmol13a} all smart meters send their masked values directly to the energy supplier (ES), which knows the sum of the shares.
If a smart meter fails, the initial exchange of the random shares must be triggered again. Lost messages are treated using acknowledgement (ACK) signals similar to \cite{Knirsch16a}, and require not only additional steps but also that the key aggregator and the ES do not collude.
%The random shares are then updated in each round by the help of a smart meter that is assigned as key aggregator for a given time period. 

In the context of federated learning with sensitive data \cite{Bonawitz17a}, masking is combined with secret sharing to handle dropping users. In this case, a recovery round is needed, and a second masking procedure is applied to preserve privacy of the dropping users in the recovery phase.
Secure multiparty computation using threshold Shamir secret sharing with fault-tolerance is proposed in \cite{Mustafa19a}. While computations for smart meters are cheap, most computations are done at DCCs (Data Communication Companies). 
%Using a suitable protocol collusion are not successful as long as there is at least one honest computational party. 
Trust in the DCCs is needed, since  %considering the present trading of collected costumer data 
privacy is not guaranteed if all DCCs collude.

In all these papers, fault tolerance needs additional effort or trust in additional parties. Only in \cite{Knirsch16a}, aggregation can be done in presence of failures without any of these requirements. However, some failures are only detected but not handled, and may lead to incomplete rounds (see Section \ref{sec:improveFailureResistance}). %However, the protocol suffers from some issues that are described next. After solving these issues the algorithm is developed further by simplifying the flow and enabling the use of homomorphic encryption. 


==> variousLengths/improveFailResistLong.tex <==
\begin{figure}[htb]
	\centering
	\input{tikz/tikzNetwork2.tikz}
\caption{Example network consisting of 5 smart meters and the data concentrator used to demonstrate assumptions, algorithms and arising problems. Connections that are on and off at round $t$ are solid and dashed, respectively. Smart meters that will get active are filled, used links are green, unused links are black.}
\label{fig:exNetwork0}
\end{figure}
%Before analyzing the existing algorithm some useful terms are introduced. 
The improved Algorithm \ref{fig: algoGeneralV02} is designed to proceed from the $\DC$ along the ring of smart meters and back to the $\DC$. During proceeding along the ring, a party is \textit{active}, does some computations and then activates the next party in the list. Only acting in the initialization part (especially line 2) is not considered as active. 
Due to malfunctions not all smart meters will be available. A party is called \textit{reachable}, if it can be reached from the currently active party. A smart meter $\SM_j$ will be called \textit{contributing} at round $t$, if its measurement will contribute to the aggregate of the measurements at round $t$.

\input{tikz/algoGeneralV02.tex}

%The existing algorithm does not clearly state the assumptions under which the algorithm terminates properly. 
% For a better understanding of the algorithms and possible problems the example network shown in Figure \ref{fig:exNetwork0} is used throughout the paper. 
%The network also reflects the assumption that the status of a link does not change within an aggregation round. 
Now failure resistance of algorithm \ref{fig: algoExisting} is discussed. Two basic types of non-working (dashed) links can occur: either links between two subsequent smart meters 
%(here $\SM_3$ and $\SM_4$, so $\SM_4$ is not reachable from the active party $\SM_3$) 
or links between a smart meter and the $\DC$ can be off.
First, consider failures of links between subsequent smart meters like between $\SM_3$ and $\SM_4$ in Figure \ref{fig:exNetwork0}. The existing algorithm does not clearly state the assumptions under which the algorithm terminates properly.  For example, this link could only work in forward direction or changes from on to off in the same round $t$. As a consequence it could happen that $\SM_3$ successfully sends the message $M_{3\to 4}$ to $\SM_4$ but the Ack-signal back to $\SM_3$ does not get through. Therefore both smart meters proceed: $\SM_3$ incorrectly assumes that it has not reached $\SM_4$ and will try to reach $\SM_5$ next. Smart meter $\SM_4$ incorrectly assumes that smart meter $\SM_3$ knows that it has been reached and continues with the procedure itself. Subsequently, also $\SM_4$ contacts $\SM_5$ which has no instructions for how to solve this case. The assumption that a communication link either works or not rules this situation out.



% As already described in \ref{sec:existingAlgo}, a failure in the communication from a smart meter to the $\DC$ (such as for $\SM_2$ in Figure \ref{fig:exNetwork0}) can be detected but not corrected by the $\DC$. This failure would require at least an additional round of reading.
%Thus, an additional round of reading where all links from smart meters to the $\DC$ work is needed. 
Second, consider a non-working link between a smart meter and the $\DC$. In the worst case this failure could happen for the \textit{last} active smart meter $\SM_N$. Algorithm \ref{fig: algoExisting} would then fail to terminate because this smart meter has no instruction of how to send the sum of the shares $S_N$ to the $\DC$ when this link fails. This situation is ruled out as follows: now all the smart meters send their masked measurements to the $\DC$ at the beginning of a round $t$. Instead of a full list of smart meters, the $\DC$ right at the start only includes the smart meters from which a message has been received in the sending list $\Lcand$ of \textit{remaining} smart meters (line 3). Due to our common assumption all later messages in the same round $t$ to the $\DC$ will then also get through and these failures are ruled out at later stages of the same round. This removal has no disadvantages, because the removed smart meters would also fail in sending their masked measurement to the $\DC$ and could therefore not contribute to the aggregate anyway. The simplification additionally handles the case of non-working smart meters which can of course also not send messages to the $\DC$. %the same way, can not send to the $\DC$ they are automatically handled as smart meters that and are therefore also removed from the sending list $\Lcand$ at the beginning of a round $t$ (line 3). 
The determination of the end of the round is different to Algorithm \ref{fig: algoExisting} by subsequently removing previous active and unreachable smart meters from $\Lcand$ and ending the round when $\Lcand$ is empty. 

%\input{tikz/algoGeneralV02.tex}


Note that the proof of termination heavily influenced the resulting algorithm: the termination failure above was only detected when trying to systematically prove the termination of a preliminary version of the protocol. The simplification then arose in an attempt to simplify the proof by removing case distinctions. This demonstrates the necessity and benefit of formally proving desired properties of the protocol.

% This step greatly simplifies the problem of non-working links due to the removal of the uncertainty which links to the $\DC$ might not work. 



% deals with these situations in line 27: only, if the Ack-signal gets back from the $\DC$, the smart meter actively contributes in the summation of the shares. In the case of $\SM_6$ in the example one additionally has to take care that the final end-of-round message is transmitted to the $\DC$. This is done by going back and letting the end-of-round message be sent by the last active smart meter (lines 44-53). While going back is not an elegant solution the overhead should be small for reasonable situations. 

% If the time interval between rounds gets small, the process of obtaining the measurements could take longer than this interval. Consequently, the next round $t+1$ starts before $t$ has finished. Therefore, in order to assign values to the right round, the round number is now also included in the message. From the security view the inclusion of the round number has another effect: if one specifies the function to ignore messages from past rounds, replay attacks could be made more difficult.






%% Old example network
% \begin{figure}
% 	\centering
% 	\input{tikz/tikzNetwork0.tikz}
% \caption{Example network consisting of 6 smart meters and the data concentrator used to demonstrate the algorithms and arising problems. The connections between the nodes are the links that work at round $t$.}
% \label{fig:exNetwork0}
% \end{figure}


%% Example flow old example network
% \begin{figure} 
% 	\centering
% 	\input{tikz/tikzFigNetwork.tikz}
% \caption{Example network showing the smart meters as nodes on the left and the $\DC$ at the right and all connections working at aggregation round $t$. Round smart meter nodes will be active in the algorithm, but only nodes filled with green color will contribute to the sum. White, round nodes do not contribute to the sum due to the missing link to the $\DC$. Red, rectangular nodes do not contribute to the sum since they are never active during the algorithm. As a result, some connections (marked as dashed, gray) exist but are not used during aggregation round $t$.}
% \label{fig:exampleNetwork}
% \end{figure}


% \begin{figure}
% 	\centering
% 	\input{tikz/tikzNetwork22.tex}
% \caption{New example network after simplification}
% \label{fig:exNetwork22}
% \end{figure}



==> variousLengths/improveFailResistShortOld.tex <==

%Before analyzing the existing algorithm some useful terms are introduced. 
\papertitle, as illustrated in Algorithm \ref{fig: algoGeneralV02}, is designed to proceed from the $\DC$ along the ring of smart meters and back to the $\DC$. During proceeding along the ring, when a party is \textit{active}, it performs some computations and then activates the next party in the list. Only acting in the initialization part (especially line 2) is not considered as active. Computations that do not influence the data flow are marked blue and will be specified later in Table \ref{tab:computations}.
Due to malfunctions, not all smart meters may be available. A party is called \textit{reachable}, if it can be reached from the currently active party. A smart meter $\SM_j$ is called \textit{contributing} at round $t$, if its measurement will contribute to the aggregate of the measurements at round $t$.

\input{tikz/algoGeneralV02.tex}

%The existing algorithm does not clearly state the assumptions under which the algorithm terminates properly. 
% For a better understanding of the algorithms and possible problems the example network shown in Figure \ref{fig:exNetwork0} is used throughout the paper. 
%The network also reflects the assumption that the status of a link does not change within an aggregation round. 
%Now failure resistance of algorithm \ref{fig: algoExisting} is discussed. 
Two basic types of non-working (dashed) links can occur: either links between two subsequent smart meters 
%(here $\SM_3$ and $\SM_4$, so $\SM_4$ is not reachable from the active party $\SM_3$) 
or links between a smart meter and the $\DC$ can be off. First, consider a non-working link between a smart meter and the $\DC$. In the worst case, this failure could happen for the \textit{last} active smart meter such as $\SM_4$ in Figure \ref{fig:exNetwork0}. Algorithm \ref{fig: algoExisting} would then fail to terminate because $\SM_4$ has no instruction of how to send the sum of the shares $S_4$ to the $\DC$ when this link fails.

\begin{figure}[htb]
	\centering
	\input{tikz/tikzNetworkShort}
\caption{Example network consisting of 4 smart meters and the data concentrator used to demonstrate arising problems. Connections that are on and off at round $t$ are solid and dashed, respectively.}
\label{fig:exNetwork0}
\vspace*{-2ex}
\end{figure}

Such issues are resolved by changing the flow such that all the smart meters send their masked measurements to the $\DC$ at the beginning of a round $t$. Instead of a full list of smart meters, the $\DC$ only includes the smart meters from which a message has been received in the sending list $\Lcand$ of \textit{remaining} smart meters (line 3 of algorithm \ref{fig: algoGeneralV02}). For Figure \ref{fig:exNetwork0}, this would result in $\Lcand =\{1,3\}$.  Due to our assumption, all later messages in the same round $t$ to the $\DC$ will also get through. % and these failures are ruled out at later stages of the same round. 
%This removal has no disadvantages, because 
The removed smart meters would have failed in sending their masked measurement to the $\DC$ and could therefore not contribute to the aggregate anyway. The simplification additionally handles the case of non-working smart meters. %, which can of course also not send messages to the $\DC$. 
The end of the round is now determined in a new way %to Algorithm \ref{fig: algoExisting} 
by subsequently removing previous active and unreachable smart meters from $\Lcand$ and ending the round when $\Lcand$ is empty.

The assumption that the bidirectional links are either on or off is also important for links between smart meters. As an example, assume that the link between $\SM_1$ and $\SM_2$ only works in forward direction or changes from on to off within the same round $t$. As a consequence it could happen that $\SM_1$ successfully sends the message $M_{1\to 2}$ to $\SM_2$ but the Ack-signal back to $\SM_1$ does not get through. Therefore both smart meters proceed: $\SM_1$ incorrectly assumes that it has not reached $\SM_2$ and will try to reach $\SM_3$ next. Smart meter $\SM_2$ incorrectly assumes that smart meter $\SM_1$ knows that it has been reached and continues with the procedure itself. Subsequently, also $\SM_2$ contacts $\SM_3$ which has no instructions for how to solve this case. 
While no setting like this is specified in \cite{Knirsch16a}, in this paper the termination of \papertitle will be proven in Section \ref{sec:termination}.  
Note that the proof of termination heavily influenced the resulting algorithm. %: the termination failure above was only detected when trying to systematically prove the termination of a preliminary version of the protocol. The simplification then arose in an attempt to simplify the proof by removing case distinctions. 
This demonstrates the necessity and benefit of formally proving desired properties of the protocol.

